What Matters in Building Vision-Language-Action Models for Generalist Robots

To utilize Foundation Vision Language Models (VLMs) for robotic tasks and motion planning, the community has proposed different methods for injecting action components into VLMs and building the Vision-Language-Action models (VLAs). In this work, we disclose the key factors that significantly influence the performance of VLA on robot manipulation problems and focus on answering three essential design choices: which backbone to select, how to formulate the VLA architectures, and when to add cross-embodiment data. The obtained results convince us firmly to explain why we prefer VLA and develop a new family of VLAs, RoboVLMs, which require very few manual designs and achieve a new state-of-the-art performance in three simulation tasks and real-world experiments. Through our extensive experiments, which include over 8 VLM backbones, 4 policy architectures, and over 600 distinct designed experiments, we provide a detailed guidebook for the future design of VLAs. In addition to the study, the highly flexible RoboVLMs framework, which supports easy integrations of new VLMs and free combinations of various design choices, is made public to facilitate future research. We open-source all details, including codes, models, datasets, and toolkits, along with detailed training and evaluation recipes at: robovlms.github.io.

==> papers/0-abs.tex <==
\begin{abstract}
To utilize Foundation Vision Language Models (VLMs) for robotic tasks and motion planning, the community has proposed different methods for injecting action components into VLMs and building the Vision-Language-Action models (VLAs). 
% Foundation Vision Language Models (VLMs) exhibit strong capabilities in multi-modal representation learning, comprehension, and reasoning. By injecting action components into the VLMs, Vision-Language-Action models (VLAs) can be naturally formed and also show promising performance. Existing work has demonstrated the effectiveness and generalization of VLAs in multiple scenarios and tasks. Nevertheless, the transfer from VLMs to VLAs is not trivial since existing VLAs differ in their backbones, action-prediction formulations, data distributions, and training recipes. This leads to a missing piece for a systematic understanding of the design choices of VLAs. 
In this work, we disclose the key factors that significantly influence the performance of VLA \minghuan{on robot manipulation problems} and focus on answering three essential design choices: which backbone to select, how to formulate the VLA architectures, and when to add cross-embodiment data. The obtained results convince us firmly to explain why we prefer VLA and develop a new family of VLAs, RoboVLMs, which require very few manual designs and achieve a new state-of-the-art performance in three simulation tasks and real-world experiments. Through our extensive experiments, which include over 8 VLM backbones, 4 policy architectures, and over 600 distinct designed experiments, we provide a detailed guidebook for the future design of VLAs. In addition to the study, the highly flexible RoboVLMs framework, which supports easy integrations of new VLMs and free combinations of various design choices, is made public to facilitate future research. We open-source all details, including codes, models, datasets, and toolkits, along with detailed training and evaluation recipes at: \url{robovlms.github.io}.

% In recent years, foundation \textit{Vision Language Model}s (VLMs) have demonstrated strong capabilities in multi-modal representation learning, comprehension, and reasoning. Building generalist robotic policies, i.e., \textit{Vision-Language-Action Models} (VLAs), have become a natural extension by injecting action components into the VLMs. Existing work has demonstrated the effectiveness and generalization of VLAs in multiple scenarios and tasks. Nevertheless, as existing VLAs differ in their backbones, action-prediction formulations, data distributions, and training recipes, a systematic understanding of the design choices of VLAs remains a missing piece of the VLA research.
% In this work, we conduct a comprehensive empirical study with extensive experiments over different VLA design choices, and introduce a new family of VLAs, \textit{RoboVLMs}, which have minimal manual designs and achieve a new state-of-the-art performance in three simulation tasks and real-world experiments.
% Specifically, our study focuses on answering three essential design choices: {\bf which} backbone to select, {\bf how} to formulate the VLA architectures, and {\bf when} to add cross-embodiment data. Through our extensive experiments, which include over 8 VLM backbones, 4 policy architectures, and over 600 distinct designed experiments, we provide a detailed guidebook for the future design of VLAs. 
% In addition to the study, the highly flexible RoboVLMs framework, which supports easy integrations of new VLMs and free combinations of various design choices, is made public to facilitate future research.
% We open-source all details, including codes, models, datasets, toolkits, along with detailed training and evaluation recipes at: \url{robovlms.github.io}.
\end{abstract}

==> papers/1-intro.tex <==


\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.9\textwidth}
        \includegraphics[width=\linewidth]{imgs/formulation_ill.pdf}
        \caption{The illustration of \red{strategies of learning-based robot policies. The existing robot policies can be categorized into the following four classes: Model-Free Learning, Model-Based Learning, World Model Based Learning, and Vision-Language-Action Model. The former three formulations consider the language-conditioned manipulation in different manners: Model-free Learning encodes the state into latent variables and utilizes a task-specific policy network to predict the action. Model-based learning solves the manipulation problem by decomposition. Yet, for tasks with complex dynamics (e.g., opening doors or cutting apples), an accurate dynamics model is demanded, while it is extremely hard to learn and generalize.  World-model-based learning predicts the goal states (e.g., the goal image) and predicts actions accordingly. While the vision-language-action model is a specific branch of model-free learning, which fully exploits the generalization and robustness of vision-language models (VLMs), and utilizes VLMs as the state encoder, facilitating strong performance on unknown object semantics and instruction following.
        }}
        \label{fig:ill_why}
    \end{subfigure}
    % \hfill
    \begin{subfigure}{0.9\textwidth}
        \includegraphics[width=\linewidth]{imgs/exist_works_new.pdf}
        \caption{The structure categorization of the existing generalist policies and recent works, based on two primary levels: 1) action space (vertical axis); and 2) whether the history information is integrated (horizontal axis). Moreover, for the VLAs that involved history, we split the VLAs that involved history into policy head and interleaved formulation based on the organization pattern of the history information. Note that this categorization not only considers models derived from pre-trained VLMs but also encompasses policy architectures that, while not pre-trained on VLMs (and therefore not claimed as VLAs), can provide insights into transforming VLMs into VLAs. Note that the works lied in the gray circle refer to the VLMs-based VLAs.
        }
        \label{fig:texonomy}
    \end{subfigure}
    \caption{The strategies of learning-based robot policies and the categorization and the recent generalist policies.}
    \label{fig:exist_works}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{imgs/illustrate.jpeg}
    \caption{
    \minghuan{This work mainly considers three key ingredients for building VLAs based on VLMs: {\bf How} to formulate the problem modeled by VLAs (\textit{i.e.}, observation horizon, action space, and how to aggregate history knowledge); {\bf Which} backbone to use (\textit{i.e.}, various VLM structures, and the data scaled used for the VLM training); and {\bf When} to use extra data source to improve the VLA performance in the tested scenario (\textit{e.g.}, in domain robot data on different tasks, and cross-embodiment data). With our proposed \textit{RoboVLMs}, we can easily transfer various VLMs into generalist robot policies, while supporting multiple embodiments, scenarios, and tasks.}
    }
    \label{fig:illustration}
\end{figure}

\section{Introduction}
\label{sec:intro}

Building generalizable robot policies capable of perceiving, reasoning, and interacting with the physical environment given human instructions has been a long-standing challenge in robotics~\citep{bousmalis2023robocat,brohan2023rt,black2024pi_0,o2023open, liu2025embodied}.
\red{Recently, there has been an active exploration of \textit{Vision-Language-Action Models} (VLAs), namely, a family of learning-based robot foundation models directly built upon generalist \textit{Vision-Language Models} (VLMs),
and they have demonstrated promising results of semantic generality} in both simulated and real-world tasks~\citep{brohan2023rt,kim2024openvla,li2023vision} (Although the rigorous definition of VLAs is not consistent in different works, we regard the ones directly built upon large-scale VLMs along with robot-domain data as the key factor to identify VLAs in this work.).
\textcolor{black}{As shown in Fig.~\ref{fig:ill_why}, existing robot policies can be categorized into four main groups:
(1) \textbf{Model-Free Learning}, which encode the state into a latent representation and use a policy network to predict actions, enabling generalization across different embodiments;
(2) \textbf{Model-Based Learning}, which rely on the robot's affordances and explicit models of the robot and environment, limiting their applicability to specific configurations;
(3) \textbf{World Model Based Learning}, which predicts future goal images and derives actions via inverse dynamics models; and
(4) \textbf{Vision-Language-Action (VLA) Model}, representing a specialized branch of model-free learning that leverages the generalization and robustness of Vision-Language Models (VLMs) by employing them as state encoders.}
Therefore, a natural question arises: \textbf{Why} do we prefer \textbf{VLA}s built upon large-scale pre-trained VLMs?
As shown in Fig.~\ref{fig:ill_why}, VLA is a newly raised model-free learning framework that receives natural language instruction as input and learns a generalist policy, rather than task-specific policies in traditional model-free learning. The widely-believed reason is that VLAs may inherit the \red{power} of VLMs, which have been shown powerful in learning generalized and robust representations of multi-modal data, such as text, images/videos, through extensive training on web-scale data. 
Such capabilities can facilitate the adaptation of robot foundation models to \gray{bridge the gap between} highly diverse open-world scenes \red{with} limited robotic data. 
\gray{The VLAs built upon VLMs could exhibit strong robustness and generalization over novel scenarios.}
\minghuan{However, it remains an open problem how large-scale vision-language pre-training facilitates generalist robot policies.}

While VLAs have shown early promise, effectively transferring pre-trained VLMs into high-performing robot policies remains non-trivial. Challenges still remain in how to sufficiently and efficiently select and utilize: 1) vision-language backbones; 2) formulation that best leverages multi-modal representations; and 3) the increasing robot data. As shown in Fig.~\ref{fig:illustration}, to address these challenges, we focus on three critical questions: 

\red{\textbf{1. Which kind of VLM backbones are suitable for VLAs?}}
\red{Selecting an appropriate VLM backbone is a fundamental yet underexplored design choice in adapting vision-language models for robotic control.}
\red{Modern VLMs vary widely in architecture. They differ in model capacity, visual encoder structure, fusion mechanisms, and data scale.}
\red{While these models are originally trained for general vision-language tasks, their effectiveness in policy learning depends on how well they can encode physical object properties, spatial relationships, and task-relevant semantics.}
\red{Existing works are based on diversified VLM structures, and most of them show promising results on adaptation to diverse and complicated manipulation skills.}
\red{Yet, there is no comprehensive study on how backbone choices impact downstream robot manipulation performance, and hence, it remains an open problem: Which kind of VLM backbones facilitates the VLA learning most.}

% Generalizable robot policies that can perceive, reason, and act in the physical world from human instructions remain an open challenge in robotics~\citep{bousmalis2023robocat,brohan2023rt,black2024pi_0,o2023open,liu2025embodied}.
% Recently, Vision-Language-Action Models (VLAs), defined as robot foundation models built on generalist Vision-Language Models (VLMs), have shown strong semantic generalization in both simulation and the real world~\citep{brohan2023rt,kim2024openvla,li2023vision}\footnote{We define VLAs as models directly built upon large-scale VLMs combined with robot-domain data.}.
% As illustrated in Fig.~\ref{fig:ill_why}, existing robot policies fall into four main groups:
% (1) Model-Free Learning, encoding state into latent features for direct policy prediction and embodiment generalization;
% (2) Model-Based Learning, relying on explicit robot and environment models, thus limited to specific setups;
% (3) World-Model Learning, predicting future goal images and inferring actions through inverse dynamics; and
% (4) Vision-Language-Action Models, a branch of model-free learning that leverages VLMs as state encoders for greater generalization and robustness.
% A natural question arises: Why favor VLAs built on large-scale pre-trained VLMs?
% As shown in Fig.~\ref{fig:ill_why}, VLAs learn generalist policies from natural-language instructions rather than task-specific ones. Their strength likely comes from inheriting the representational power of VLMs, which learn robust multimodal features from web-scale text–image data.
% Such representations enable robot foundation models to adapt to diverse, open-world scenes with limited robotic data, yielding robustness and generalization to novel scenarios.
% However, it remains unclear how large-scale vision–language pre-training facilitates such generalist robot behavior.


\red{\textbf{2. How should VLAs be formulated to best leverage VLMs?}} Beyond the diversity of different backbones, for generalist robot policies, including VLAs, the structures are more complex and vary in form. Based on the most prevalent existing work~\citep{li2023vision, team2024octo, wu2023unleashing, brohan2023rt, kim2024openvla, o2023open, nair2022r3m, jiang2022vima, zhen20243d, black2024pi_0}, we propose a categorization based on 1) how the history and action information are incorporated in VLAs and 2) whether the action space is continuous or discrete.
As shown in Fig.~\ref{fig:texonomy}, four types of structure formulations are considered. For history information modeling, two forms are identified: 1) \emph{one-step modeling}, which utilizes only the current state or observation to produce actions; and 2) \emph{history modeling}, which processes a sliding window of historical states or observations. Regarding the aggregation of history information, we classify it into two approaches: a) \emph{interleaved modeling}, which integrates historical observation and action sequences in an interleaved format; and b) \emph{policy head}, which separately processes each historical step and fuses the information at a distinct policy head for action prediction.
\textcolor{black}{These above-mentioned formulations leverage the pre-trained VLMs in their different ways}. Hence, they may have different features in terms of robustness, generalization ability, and data efficiency when faced with \textcolor{black}{various} types of environments and tasks. Therefore, it is practically important but underexplored to understand: How should we formulate VLAs to sufficiently leverage the power of VLMs in practice?

\red{\textbf{3. When should we leverage the public diverse robot data for optimal training?}} In addition to the VLA itself, the quality and diversity of the training data used to develop VLAs are equally critical. With recent progress achieved by well-known VLAs~\citep{team2024octo, brohan2023rt, kim2024openvla, o2023open, black2024pi_0}, large-scale data from different embodiments (also known as cross-embodiment data) is important to further improve performance in terms of robustness and generalization against out-of-distribution tasks and environments. Yet, \minghuan{they differ largely in detailed training recipes: some utilize cross-embodiment data to 1) pre-train a foundation VLA from VLMs by refining representations closer to robotic manipulation tasks~\citep{black2024pi_0, zhou2025vision} and 2) post-train the VLA with in-domain data; while others co-train VLAs with cross-embodiment data alongside in-domain data~\citep{team2024octo,brohan2023rt,kim2024openvla,o2023open}. Moreover, by being sufficiently pre-trained on cross-embodiment datasets, VLAs are expected to learn new skills with minimal demonstrations~\citep{finn2017model}.}
Consequently, in the case of developing efficient VLAs, when to leverage the large-scale cross-embodiment data becomes an intriguing issue.


To thoroughly study the aforementioned key questions,  
we propose a general framework, {\bf RoboVLMs}, to easily transfer the VLMs into VLAs and implement a fair comparison. We evaluate these models on two popular robot manipulation benchmarks in simulation: \textbf{CALVIN}~\citep{mees2022calvin} and \textbf{SimplerEnv}~\citep{radosavovic2023real}.
Moreover, we also trained and evaluated the built VLAs on a real-world robot manipulation dataset, consisting of 100 manipulation tasks and a total of 74K trajectories.
Specifically, we initially selected three commonly used VLMs--LLaVA, Flamingo, and KosMos, as backbones, combining each with the four VLA structures illustrated in Fig.~\ref{fig:texonomy} to examine the effects of action space, observation horizon, and history aggregating methods.
With the finding that the policy head modeling with continuous action space performs best, we compare 8 various VLMs as the backbone with policy head formulation to answer which backbone is more suitable. Meanwhile, we compare the generalization and data efficiency of different VLA structures. For the question of when to leverage cross-embodiment data, we compare co-training (the VLAs trained with Open X-Embodiment), finetuning (the VLAs trained with the target dataset), and post-training (the VLAs co-trained with Open X-Embodiment and further finetuned with the target dataset). Finally, to confirm the real-world applicability of the VLAs with the optimal configuration, we trained and evaluated them in real-world robot manipulation scenarios, demonstrating generalization across 1) unseen distractors, 2) unseen backgrounds, 3) unseen target objects, and 4) novel skill descriptions.

Through our extensive and comprehensive studies, we derive conclusions on how to build high-performance VLAs around the following questions:

\noindent{\bf Why do we prefer VLAs?} 
VLAs built upon pre-trained VLMs have proven to be both effective and efficient for generalist robot policies. Across all experiments, including simulations and real-world manipulation tasks, our VLA consistently outperforms open-source state-of-the-art VLAs by a significant margin. Furthermore, pre-trained VLMs exhibit notable advantages in generalization and data efficiency, making them highly desirable for real-world robotic applications.

\noindent{\bf Which VLM backbone is more suitable for VLAs?}
Our extensive study on 8 different VLM backbones shows two distinguished VLM backbones, namely KosMos~\citep{peng2023kosmos} and Paligemma~\citep{beyer2024paligemma}, which significantly outperform the others. These results highlight that comprehensive vision-language pretraining is essential for achieving superior VLA performance.

\noindent{\bf How should we formulate VLAs?}
Through extensive study and experiments, continuous actions consistently outperform auto-regressive discrete actions, while incorporating historical context is crucial for enhancing performance and addressing partial observability.
For the model architecture, Vision-Language Models (VLMs) integrated directly with policy heads demonstrate superior performance compared to other formulations due to the consistent usage, i.e., vision-language tokens should be processed in their original pretraining format, with a policy head added to integrate past visual and proprioceptive observations for effective decision-making.
Finally, larger VLMs further enhance efficiency, requiring fewer data to achieve higher performance.

\noindent{\bf When should we leverage cross-embodiment datasets?} 
While it is widely believed that pre-training or post-training with cross-embodiment data improves performance, this belief has not been rigorously validated. Our findings reveal that pre-training with cross-embodiment data does not consistently yield significant improvements in final performance. However, post-training a cross-embodiment pre-trained model on the target dataset can lead to notable performance gains. Additionally, leveraging manipulation data from the same robots or tasks provides a clear boost in performance.

\gray{Throughout the study, we propose a new framework, {\bf RoboVLMs}, which transfers VLMs into VLAs, and provides a unified, flexible, easy-to-use, open-source framework that enables seamless integration of any VLM into VLAs with minimal effort, allowing robotics practitioners to investigate, compare, and deploy future VLAs. Further, the VLAs built by RoboVLMs demonstrate strong performance in generalization, dexterity, and flexibility across a wide range of benchmarks and real-world tasks.}
\gray{We open-source the code, along with model weights, and comprehensive guidelines to facilitate the reproducibility of all the results. Our goal is to shed light on the robotics community and help build generalized robots.}


==> papers/2-results.tex <==


\section{Main Results and Findings}
\label{sec:resutls}

\gray{Vision-language-action models (VLAs) are commonly defined as models fine-tuned from pre-trained large-scale vision-language models (VLMs) using imitation learning~\citep{li2023vision,brohan2023rt}. By leveraging the robust vision-language representation capabilities of VLMs, VLAs offer a promising approach for developing generalist robotic policies capable of handling complex tasks. However, this approach is not universally accepted as the sole or optimal solution. For instance, modular approaches utilize pre-trained vision and language modules to encode latent representations of multi-modal inputs~\citep{mees2022matters,brohan2022rt}, while alternative methods rely on direct training with diverse robotic datasets~\citep{team2024octo}. Even within VLA research, there is no consensus on architectures or training recipes~\citep{li2023vision,cheang2024gr,kim2024openvla, brohan2023rt}.}

The primary objective of this work is to establish VLAs as robust generalist robotic policies by thoroughly analyzing contemporary VLA architectures and identifying the key factors driving their performance.
% \red{Concretely, we aim to answer the following questions:}
% \gray{To this end, we introduce RoboVLMs, a unified VLA framework that enables the systematic integration and exploration of essential components in VLA design. Using this framework, we conduct extensive experiments to address several critical questions.}

% \begin{enumerate}
%     \item \textbf{Why} do we prefer VLAs?
%     \item \textbf{Which} kind of VLM backbones are suitable for VLAs?
%     \item \textbf{How} should VLAs be formulated to best leverage VLMs?
%     \item \textbf{When} should we leverage the public diverse robot data for optimal training? 
% \end{enumerate}
As shown in Extended Table.~\ref{tab:chapter_split}, we aim to answer the four questions (why/which/how/when) described in the former section. The 4 questions are further divided into 6 executable research problems, and successively experiments are designed to answer each.
% The built VLA model with a proper backbone and structure can outperform the state-of-the-art generalist robot policies by a large margin. We hope that our findings can practically help build robust, generalizable, and well-performing VLAs.
% By answering these questions, we build RoboVLMs, a family of strong VLA models that outperform the state-of-the-art generalist robot policies by a large margin. We hope that our findings can practically help build robust, generalizable, and well-performing VLAs.
% With the taxonomy as discussed, we name the implemented VLAs in this work in a principle of ``\textit{Backbone} \textit{History Modeling}''

% \subsection{Benchmarks and Evaluation Metrics}
\begin{figure}[!t]
\centering
    \begin{subfigure}{0.8\textwidth}
        \centering
        \includegraphics[width=\linewidth]{imgs/exps_setup.pdf}
        \caption{Two simulated and one real-world benchmarks. We show environment setups and example tasks involved.}
        \label{fig:env}
    \end{subfigure}
    \vspace{0.5cm}
    \begin{subfigure}{0.8\linewidth}
        \centering
        \includegraphics[width=\linewidth]{imgs/robot_demo.pdf}
        \caption{The demonstration of our real robot platform. The platform is equipped with a side camera and a wrist camera. 
        }
        \label{fig:real_robot}
    \end{subfigure}
    \vspace{0.5cm}
    \begin{subfigure}{0.8\textwidth}
        \centering
        \includegraphics[width=\linewidth]{imgs/real_illustrate.jpeg}
        \caption{The illustration of the experimental settings in real-world experiments. We evaluate the models in 20 tasks with five settings for each task, involving \textsl{Unseen Disctractor}, \textsl{Unseen Target Object} and \textsl{Unseen Background}, \textsl{Novel Skill Description}. 
        % Note that for tasks like \texttt{Open Drawer}, we do not test the unseen object setting, and the object layout for each rollout is randomly initialized and different from the one in the training set. Note that the unseen target object is only available for picking tasks.
        }
        \label{fig:real_illustration}
    \end{subfigure}
\caption{Illustration of the involved simulations and real-world benchmarks.}
\label{fig:env_ill}
\end{figure}

\subsection{Benchmarks and Evaluation Metrics}

To comprehensively evaluate the performance of VLAs, in this work, we benchmark all models on a diverse set of benchmarks and robotic manipulation tasks in both simulation and the real world. Specifically, as shown in Fig.~\ref{fig:env}, we choose two well-known and widely-used simulation benchmarks ({\bf CALVIN}~\citep{mees2022calvin} and {\bf SimplerEnv}~\citep{torne2024reconciling}) as our testbed. Moreover, we deploy and test our system on a real-world robot manipulation benchmark, including more than 100 tasks, to evaluate RoboVLMs.

\textbf{CALVIN}~\citep{mees2022calvin} is a simulation benchmark for multitask table-top manipulation.  The dataset contains four splits A, B, C, and D according to different scene settings and provides 34 basic tasks with 24K human teleoperated demonstrations annotated with language instructions in total. Evaluation metrics include the success rates of finishing $1\sim 5$ consecutive tasks, as well as the average number of achieved tasks successfully executed (shortened as \textit{Avg. Len.}).
% It provides 24K human teleoperated demonstrations annotated with language instructions from 34 pre-defined basic skills, such as \texttt{Opening Drawer}, \texttt{Turning on LED}, \texttt{Stack Block}, \textit{etc}. 
% Each trajectory consists of less than 64 time steps.
% The dataset contains four splits A, B, C, and D according to different scene settings.
% During evaluation, the robot is required to complete a sequence of five consecutive tasks. 
% Evaluation metrics include the success rates of finishing $1\sim 5$ consecutive tasks, as well as the average number of achieved tasks successfully executed (shorted as \textit{Avg. Len.}).
    
\textbf{SimplerEnv}~\citep{li2024evaluating} is designed as a suite of real-to-sim environments and enables the evaluation of robot policies in simulation. It creates a comparable arena for benchmarking the success rate of robot policies in private real-world settings such as Google Robot~\citep{brohan2022rt,brohan2023rt} and Bridge V2~\citep{walke2023bridgedata}.
% It is an efficient, scalable, and informative alternative to real-world evaluation for models trained on real-world manipulation datasets.
% SimplerEnv creates a comparable arena for benchmarking robot policies in private real-world settings such as Google Robot~\citep{brohan2022rt,brohan2023rt} and Bridge V2~\citep{walke2023bridgedata}.
% To benchmark the performance on SimplerEnv, we test the success rates of our models on the above two most widely used subsets.
Evaluation metrics for SimplerEnv are the success rate of each task, simply counted by the number of successfully finished tasks over all valid trials.

\textbf{Real Robot Benchmark}~\citep{cheang2024gr} consists of over 70K teleoperated human trajectories used to fine-tune robot policies, covering 105 manipulation tasks. To evaluate the performance of models on this benchmark, we adopt the approach outlined in~\citep{li2024gr}, testing each model on one \textit{Simple} setting and four challenging \textit{Unseen} settings. Examples of these settings are shown in Fig.\ref{fig:real_illustration}. In total, we evaluate each VLA across 20 tasks, with 5 settings per task and 3 rollouts per setting, reporting the average success rate for each setting. A detailed description of the benchmarks is provided in Appendix.



% Some examples are shown in Fig.~\ref{fig:real_illustration} and Fig.~\ref{fig:real_illustration_full}.
% The evaluation includes two parts: \textit{Simple} and \textit{Unseen}.
% For \textit{Simple} evaluation, the test scenarios are set similarly to the training ones, with the same set of objects and task instructions.
% For \textit{Unseen} evaluation, it is split into four different settings: \textit{Unseen Skill}, \textit{Unseen Distractor}, \textit{Unseen Background}, and \textit{Unseen Object}.
% We follow the same definition for these settings introduced in \citet{cheang2024gr}, which can also be found in the Appendix~\ref{ap:bench_details}.
% We compare the success rate on more than 80 tasks with different objects, skills, and backgrounds.

% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=\textwidth]{imgs/real_illustrate.jpeg}
%     \caption{The illustration of the experimental settings in real-world experiments. We evaluate the models in 20 tasks with five settings for each task, involving \textsl{Unseen Disctractor}, \textsl{Unseen Target Object} and \textsl{Unseen Background}, \textsl{Novel Skill Description}. Note that for tasks like \texttt{Open Drawer}, we do not test the unseen object setting, and the object layout for each rollout is randomly initialized and different from the one in the training set. Note that the unseen target object is only available for picking tasks.}
%     \label{fig:real_illustration}
% \end{figure*}

\gray{All tasks included in these benchmarks are driven by single-arm robots, leading to a 7-DoF action - the 6D pose~\footnote{Represented in Euler angles.} of the gripper and one-dimensional open/close status. Robot observation is accessible from proprioceptive sensory information, visual observation, and language input.}

\subsection{Why do we prefer VLAs?}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{imgs/simpler_hist.pdf}
        \caption{Evaluation results on the \textbf{SimplerEnv} simulation benchmarks, including the \textit{WidowX+Bridge} and \textit{Google Robot} environments. Performance of baseline methods are referred from \citet{li2024evaluating}. The KosMos P.H. built by RoboVLMs is the best VLA structure investigated, which is trained over fixed training steps. Detailed numerical results can be further referred to Extended Table.~\ref{tab:simpler_merge}.}
        \label{fig:simpler_hist}  % ✅ 正确：放在 \caption 后面
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{imgs/calvin_novl_avg_len_comparison.pdf}
        \caption{Ablation study of VLAs for vision-language pre-training on different settings of the CALVIN benchmark. ``P.H." denotes policy head. ``No VL" suggests models without VL pre-training. ``Inter" refers to the interleaved formulation. ``5x" represents training with 5x re-generated training data. Full results on different training settings and data scales are shown in Appendix.}
        \label{fig:calvin_novl_generalization}  % ✅ 正确
    \end{subfigure}

    \begin{subfigure}[b]{0.7\textwidth}
        \includegraphics[width=\linewidth]{imgs/calvin_generalization_ablation_abcd_d.pdf}
        % \caption{Trained on split ABCD.}
        \label{fig:calvin_gen_abcd}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.7\textwidth}
        \includegraphics[width=\textwidth]{imgs/calvin_generalization_ablation_abc_d.pdf}
        \caption{Performance on \textbf{CALVIN} benchmark, all models are trained on split ABC/ABCD, and evaluated on split D (the upper figure is trained on ABC, and the lower figure ABCD). We report the success rates of five consecutive tasks (left axis) and the averaged task length (right axis), using the model checkpoint at 5\textsuperscript{th} epoch.}
        \label{fig:calvin_generalization}
    \end{subfigure}
    % \vspace{0.5cm}
    \begin{subfigure}{0.7\textwidth}
        \centering
        \includegraphics[width=\linewidth]{imgs/plot_hist.pdf}
        \caption{Real-robot performance of our best VLA (KosMos P.H.) built by RoboVLMs against baseline methods over different settings. RoboVLM outperforms the existing VLAs over all settings, especially for metrics in unseen scenarios, demonstrating the effectiveness and robustness of our model.}
        \label{fig:real_res}
    \end{subfigure}
    
    \caption{The experimental results for RoboVLMs in Simulations.}
    \label{fig:total}  % ✅ 主图的label放在主caption后面
\end{figure}


This section investigates one of the key questions: \textit{Why do we want VLAs?} To answer this question, we need to answer the following prerequisite sub-question first:
\question{1.1}{Are VLAs a proper choice for building generalist robot policies?}
Concretely, we demonstrate the best-performing VLA resulting from our study, which sets a new state-of-the-art result on both \textbf{CALVIN} and \textbf{SimplerEnv} benchmarks, outperforming all other robot policies with a clear margin.
All results are shown in Extended Table.~\ref{tab:performance_calvin} and Fig.~\ref{fig:simpler_hist}. From these tables, we can see that our strongest RoboVLM exceeds the existing state-of-the-art generalist policies by a large margin and establishes a strong baseline for robot manipulation tasks both in simulation and real-world experiments. Concretely, we can easily observe the following facts:
\begin{itemize}
    \item 
    % \textit{The best setting VLA built with RoboVLMs (KosMos P.H.) demonstrate strong generalization capabilities compared with the baselines.} 
    On \textbf{CALVIN} benchmark, our best model achieves the highest performance in all metrics and demonstrates superior generalization ability when transferring from ABC to D (a novel scene unseen in the training splits) with an absolute improvement of 12.6\% for the execution of a single task and a total improvement of 30.3\% for 5 consecutive tasks. 
    On average, under zero-shot settings, our model can finish 4.25 tasks out of 5 tasks for each single rollout, outperforming the previous SOTA model (GR-1) by 1.19 tasks.
    
    \item 
    % \textit{KosMos P.H. still exhibits stronger generalizing ability on more photo-realistic simulator.} On \textbf{SimplerEnv}, 
    % our model achieves the highest average performance on all tasks except the \texttt{Open/Close Drawer} environments, 
    On \textbf{SimplerEnv}, our model achieves the highest average performance on both \textit{WidowX + Bridge} and \textit{Google Robot} environments,
    demonstrating the general effectiveness and robustness against different settings and diverse manipulation tasks.

\end{itemize}


We also investigated the impact of vision-language pre-training on the generalization and data efficiency (Fig.~\ref{fig:calvin_novl_generalization} and Extended Table.~\ref{tab:data_eff_calvin}).
For the generalization in CALVIN, we adopt the official setting: training models on the split of ABC and validating performance on D. 
To evaluate data efficiency, we conduct experiments on model scales ranging from 3B to 9B and various data scales: 10\% training data (\textbf{0.1x ABCD}), the standard setting (\textbf{ABCD}), and 500\% training data (\textbf{5x ABCD}). The additional data originates from the officially released unlabeled datasets, following the setups as introduced in \citet{wu2023unleashing}. The detailed results on different data scales are shown in Appendix.

We can see that vision-language pre-training is essential for both generalization and data efficiency. This observation is intuitive, as an aligned vision-language representation provides a robust foundation for visual understanding, enabling the policy to focus on learning manipulation skills.
Therefore, we can conclude that
\finding{1.1}{VLA is a promising path to generalist robot policies.}

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}{0.95\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{imgs/plot_hist.pdf}
%         \caption{Real-robot performance of our best VLA (KosMos P.H.) built by RoboVLMs against baseline methods over different settings. RoboVLM outperforms the existing VLAs over all settings, especially for metrics in unseen scenarios, demonstrating the effectiveness and robustness of our model.}
%         \label{fig:real_res}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[b]{1.0\textwidth}
%         \includegraphics[width=1.0\textwidth]{imgs/real_correction_1.jpeg}
%         % \caption{}
%         \label{fig:real_correction_sub1}
%       \end{subfigure}
%       % \vspace{-4mm} % 手动调整为负值
%       \\[-3mm] % 调整为合适的负间距
%       % 中间的子图
%       \begin{subfigure}[b]{1.0\textwidth}
%         \includegraphics[width=1.0\textwidth]{imgs/real_correction_2.jpeg}
%         \caption{Visualization for rollouts that the best setting VLA built by RoboVLMs emerges the ability of self-correction. For instance, in the \texttt{Open The Oven} task, the robot's first attempt does not reach the oven handle, and it adjusts the end-effector position to re-locate the handle at the second attempt. Note that the training dataset does not contain this kind of data.}
%         \label{fig:real_correction_sub2}
%   \end{subfigure}
%     \caption{The quantitative and qualitative results for real world experiments.}
%     \label{fig:total}  % ✅ 主图的label放在主caption后面
% \end{figure}

However, although VLAs perform well in simulation, it is still an open problem whether VLAs are suitable for real-robot applications due to the sim-to-real gap \citep{zhao2020sim}. We propose the second open question:
\question{1.2}{How does the best VLA built with RoboVLMs perform in real-world scenarios?}
As discussed above, we deploy the best-performing RoboVLM model, that is, the one based on the decoder-only KosMos in real-world scenarios to validate its effectiveness.
As shown in Fig.~\ref{fig:real_illustration}, our experiment involves 20 tasks with multiple skills, including \texttt{Open}, \texttt{Close}, \texttt{Press Button}, \texttt{Pick \& Place}, etc. For each task, we evaluate five settings, with the basic setting, novel skill description, unseen distractors, unseen target object, and unseen background.

Our robot system for real experiments is built on a 7-DoF Kinova Gen3 robot arm paired with a Robotiq 2F-85 gripper. Please refer to Sec.~\ref{sec:method} for more details of the real robot. 
For input, we take the RGB images for the two cameras equipped on the robot head and wrist separately. The head camera provides an overview of the workspace while the gripper camera offers a close observation of the interaction area between the end effector and the environment.

We fine-tune Octo-Base, OpenVLA, and KosMos P.H. built by RoboVLMs on the real robot benchmark and compare their performance. The result is shown in Fig.~\ref{fig:real_res}. We observe that the best VLA (KosMos P.H.) built by RoboVLMs achieves the best performance in all evaluation setups, especially on \textit{Simple} and \textit{Unseen Background}, demonstrating their effectiveness and generalization ability, which is consistent with the results in SimplerEnv and CALVIN simulation.

The qualitative results are shown in Appendix, including success rollouts in various settings and some representative failure cases.
KosMos P.H. not only outperforms baseline models in basic setting tasks like \texttt{Open Drawer}, \texttt{Pickup Eggplant} and \texttt{Press the Toaster Switch}, but also achieves better performance over unseen objects, distractors, and backgrounds. Furthermore, as shown in Extended Fig.~\ref{fig:real_correction}, KosMos P.H. emerges with self-correction ability, it can realize the incorrect positions of the end effector and correct its future trajectory to complete the task successfully. Note that this ability does not appear in the other tested baselines, and this kind of data is not contained in the training dataset.

\finding{1.2}{The best setup VLA built by RoboVLMs appears to have strong effectiveness and robustness in real scenarios.}

In the following, we will explain our empirical studies and corresponding findings in detail, including the settings, results, and takeaways in building VLAs from pre-trained VLMs.

\subsection{Which kind of VLM backbones are suitable for VLAs?}


% Following such a finding, the choice of using a policy head for history fusion in VLA can be finalized. 
% However, a critical question remains when selecting the most appropriate VLM to build our VLA:
When building a VLM-based VLA, the first question is which VLM backbone is the most appropriate one for our VLA:
\question{2}{Which type of VLMs is most suitable for constructing VLAs?}

To thoroughly investigate this question, it would be ideal to conduct experiments in highly controlled settings. However, training VLMs on large-scale vision-language datasets is extremely resource-intensive. Therefore, we base our VLAs on a diverse set of off-the-shelf, pre-trained, large-scale vision-language backbones with varying architectures, training data scales, model sizes, and latent embeddings. These include Flamingo model family~\citep{alayrac2022flamingo} (Encoder-Decoder), and a series of decoder-only VLMs, including LLaVA~\citep{liu2024visual}, Qwen-VL~\citep{bai2023qwen}, MoonDream~\citep{moondream}, UForm~\citep{uform-gen}, Paligemma~\citep{beyer2024paligemma}, and KosMos~\citep{peng2023kosmos}. 
Noticeably, in this section, for fair comparisons, all the models are trained with static images instead of both static and hand cameras.

\gray{Although this approach may not offer a fully controlled comparison, our extensive experiments aim to provide insights into the impact of different VLM backbones on VLAs.}
The results, presented in Extended Table.~\ref{tab:calvin_backbone}, reveals the following observation:
% \begin{itemize}
KosMos and Paligemma demonstrate the distinctively better performance. From Extended Table.~\ref{tab:calvin_backbone}, we can see that these two backbones are much better than others with a significantly clear margin. Their superior performance benefits from sufficient vision-language pre-trained on large vision-language datasets. This outcome is intuitive, as extensive pretraining facilitates stronger alignment between visual and linguistic features, an alignment critical for language-conditioned manipulation tasks.

    % \item \textbf{It is still unclear and an open problem how other factors affect the VLA performance}: Different VLMs have different kinds of training data, architecture, model size, data scale, LLM backbones, training recipes, etc. Nevertheless, the selected 8 VLM backbones are insufficient to reveal the relationships between these important components of a pre-trained VLM and VLA. It will be a valuable future direction to further investigate such relationships.
    
% \end{itemize}
\gray{We discuss more influencing factors and interesting findings in Sec.~\ref{sec:discuss}.}
\finding{2}{
% KosMos and Paligemma are distinctively better than other VLMs in terms of training VLAs. We hypothesize they benefit from sufficient vision-language pretrain.
VLAs benefit from sufficient vision-language pre-training on larger vision-language datasets of VLMs backbone.
}

\subsection{How should VLAs be formulated to best leverage VLMs?}
\label{sec:how}

In this section, our study addresses questions regarding VLA formulations, including different design choices of VLA structures and various backbones. To answer these questions, we conduct a series of controlled experimental studies to evaluate various VLA formulations on the CALVIN benchmark for rapid evaluation.


\question{3.1}{How to select the best-performing VLA structure?}

\noindent More specifically, how should we model observations, states, and actions in robot manipulation tasks within the context of a VLA? To explore this question, we implement several variants, leveraging various open-source VLM backbones such as OpenFlamingo~\citep{o2023open}, LLaVA~\citep{liu2024visual}, and KosMos~\citep{peng2023kosmos}. These variants incorporate different historical information modeling strategies, and action spaces, as discussed and categorized in Sec.\ref{sec:intro}.


\begin{table*}[!t]
\caption{The ablation study on \textbf{CALVIN} benchmark over the effect of action space, history integration, and history organizing format. All variants are trained on split ABCD and tested on split D. ``Disc." is short for discrete and ``Cont." represents continuous action space. 
% Results are reported with the best-behaved model checkpoints within 5 epochs trained on the ABCD training splits.
Note that for VLAs with LLaVA backbone, we utilize a perceiver resampler to downsample its vision tokens to 64 for fair comparison.
Results are reported with models trained maximally within 5 epochs on the ABCD training splits, all structures predict an action chunk with size 10 and only execute the first step action for inference.
}
\centering
% \begin{tabular}{l|cc|ccccc|c}
\begin{tabularx}{\textwidth}{l|>{\centering\arraybackslash}X>{\centering\arraybackslash}X|>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X|>{\centering\arraybackslash}X}
\toprule
\multirow{2}{*}{Backbone} & \multirow{2}{*}{Structure} & \multirow{2}{*}{\makecell{Action\\Space}} & \multicolumn{5}{c|}{Consecutive tasks success rates} &  \multirow{2}{*}{\makecell{\textit{Avg.}\\\textit{Len.}}} \\ \cmidrule{4-8}
 &  &  & 1 & 2 & 3 & 4 & 5 &  \\ \midrule
\multirow{4}{*}{LLaVA} & One-Step & Disc. & 0.809 & 0.484 & 0.278 & 0.175 & 0.103 & 1.85 \\
 & One-Step & Cont. & 0.793 & 0.592 & 0.420 & 0.329 & 0.235 & 2.37 \\
 & Interleaved & Cont. & {\bf 0.892} & 0.645 & 0.436 & 0.282 & 0.181 & 2.44\\
 & Policy-Head & Cont. & 0.873 & {\bf 0.678} & {\bf 0.506} & {\bf 0.376} & {\bf 0.275} & {\bf 2.71} \\ \midrule
% Qwen & One-Step & Disc. &  &  &  &  &  &  \\
% Qwen & One-Step & Cont. &  &  &  &  &  &  \\
% Qwen & Interleaved & Cont. &  &  &  &  &  &  \\
% Qwen & Policy-Head & Cont. &  &  &  &  &  &  \\
% \midrule
\multirow{3}{*}{Flamingo} & One-Step & Disc. & 0.681 & 0.318 & 0.133 & 0.062 & 0.029 & 1.22 \\
 & One-Step & Cont. & 0.681 & 0.354 & 0.158 & 0.076 & 0.035 & 1.30 \\
 & Policy-Head & Cont. & {\bf 0.964} & {\bf 0.896} & {\bf 0.824} & {\bf 0.740} & {\bf 0.662} & {\bf 4.09} \\
\midrule
\multirow{4}{*}{KosMos} & One-Step & Disc. & 0.424 & 0.097 & 0.023 & 0.005 & 0.002 & 0.55 \\
& One-Step & Cont. & 0.935 & 0.868 & 0.814 & 0.768 & 0.702 &  4.09 \\
& Interleaved & Cont. & {\bf 0.987} & 0.915 & 0.824 & 0.737 & 0.660 & 4.12 \\
& Policy-Head & Cont. & 0.967 & {\bf 0.930} & {\bf 0.899} & {\bf 0.865} & {\bf 0.826} & {\bf 4.49} \\ 
\midrule
\multirow{4}{*}{PaliGemma} & One-Step & Disc. & 0.316 & 0.096 & 0.021 & 0.005 & 0.001 & 0.44  \\
& One-Step & Cont. & 0.933 & 0.863 & 0.808 & 0.751 & 0.688 & 4.04   \\
& Interleaved & Cont. & 0.949 & 0.896 & 0.851 & 0.803 & 0.754 & 4.25 \\
& Policy-Head & Cont. & {\bf 0.984} & {\bf 0.933} & {\bf 0.888} & {\bf 0.835} & {\bf 0.779} & {\bf 4.42} \\ 
\bottomrule
\end{tabularx}
\label{tab:alblation_calvin}
\end{table*}

The performance of various VLA structures in CALVIN is summarized in Table.~\ref{tab:alblation_calvin}. From these results, we draw the following key observations:

\begin{itemize}
    \item \textbf{Continuous action matters:} By comparing two types of action spaces, {\bf continuous} and {\bf discrete}, as shown in Table.~\ref{tab:alblation_calvin}, we observe that under the single-frame formulation, continuous action spaces consistently outperform discrete ones, particularly as task horizons increase. This finding is intuitive: continuous actions can represent high-precision floating-point values, whereas discrete actions are limited to indexing action intervals. For long-horizon tasks, the accumulation of compounding errors significantly degrades the performance of discrete actions.
    
    \item \textbf{History observation matters:} As shown in Table.~\ref{tab:alblation_calvin}, under the same VLM structure (either Encoder-Decoder or Decoder-only), models incorporating history observations as input consistently outperform one-step models, achieving substantially higher success rates across all tasks. This improvement holds regardless of the history fusion strategy used. Furthermore, increasing the length of an observable history can enhance performance, albeit at the cost of higher computational overhead.
    
    \item \textbf{Policy head improves history fusion:} Among the formulations utilizing history, the interleaved history formulation performs worse than merging history via an additional policy head. We hypothesize that the policy head preserves the VLM's original vision-language fusion capabilities while effectively integrating historical information. Moreover, the interleaved formulation incurs significantly higher memory and FLOP costs during both training and inference. This suggests that incorporating history with an additional policy head is a more effective and efficient approach for VLAs.

\end{itemize}

\finding{3.1}{The VLA achieves its best performance when using multi-step historical observations as inputs and continuous actions as outputs. For integrating history with continuous action space, the policy head structure performs better.}

However, beyond the performance itself, one of the most important challenges for modern VLAs is achieving generalization to novel objects and environmental settings, which is critical for practical deployment across various robots and scenarios. Conversely, when generalization is insufficient, fine-tuning the policy with a few new demonstrations becomes ideal. Thus, VLAs should inherit the generalization capabilities of VLMs in open-world settings while maintaining high data efficiency when additional in-domain training samples are available. 

Therefore, we further investigate the generalization and data efficiency for different VLAs formulations.

\question{3.2}{How do different formulations affect the generalization and data efficiency for VLAs?}


To address the question, we empirically study and evaluate the generalization and data efficiency of various VLA formulations, aiming to provide practical insights for training high-performing VLAs.
Specifically, we assess the generalization and data efficiency of different VLAs built with RoboVLMs by training models with different architectures and formulations on varying data scales using the CALVIN datasets.
As discussed earlier, we focus on comparing the interleaved and policy head formulations using the OpenFlamingo and KosMos backbones, which have shown strong potential among all configurations. Note that the interleaved formulation can only be paired with a decoder-only structure. The results presented in Fig.~\ref{fig:calvin_generalization} and  Extended Table.~\ref{tab:data_eff_calvin}, lead to the following observations:

\begin{itemize}
    \item \textbf{For generalization performance} (Fig.~\ref{fig:calvin_generalization}), our best model, based on the KosMos backbone and leveraging a policy head for history fusion, exhibits only a slight performance drop in zero-shot settings. In contrast, other formulations experience significant performance declines. This finding highlights that the model architecture significantly impacts generalization. This conclusion is further supported by results in Fig.~\ref{fig:simpler_hist}, where tasks in the evaluation set are paired with novel instructions, and Fig.~\ref{fig:real_res}, where our best model outperforms others by a large margin across all unseen tasks.

    \item \textbf{For data efficiency,} we observe trends similar to those for generalization. Our best model consistently achieves the highest performance when training data is scaled down, with a notably slower performance decline compared to other formulations. Additionally, comparisons of encoder-decoder VLAs at different scales reveal that larger models tend to be more data efficient.

\end{itemize}

\finding{3.2}{Leveraging policy head for history fusion is the best in terms of generalization and data efficiency.}

\begin{table*}[!t]
    \centering
    \caption{The performance of VLAs with different training objectives and action execution paradigms, and whether to introduce the MoE structure. We utilize PaliGemma, which aligns with the settings of $\pi$ series, as the VLM backbone and implement Fully Connecting (FC) with MSE and Flow Matching (FM) loss. Note that the FC with Flow Matching loss and MoE structure is identity with $\pi_0$, and for fair comparison, we do not consider state as input. For executing paradigms, we verify three different paradigms: {\bf Chunk} represents that the VLAs execute the entire chunk. {\bf First} refers to VLAs execute the first action in the chunk. {\bf Ensemble} refers to ensemble the first action with the corresponding actions in history chunks.}
    \label{tab:combined1}
    
    \begin{subtable}{\textwidth}
        \centering
        \caption{Performance with different training objectives and execution paradigms}
        \begin{tabularx}{\textwidth}{l@{\extracolsep{\fill}}|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X|>{\centering\arraybackslash}X} 
\toprule
\multirow{2}{*}{\makecell{Training\\Objective}} & \multirow{2}{*}{\makecell{Training\\Split}} & \multirow{2}{*}{\makecell{Executing\\Paradigm}} & \multicolumn{5}{c|}{Consecutive tasks success rates} & \multirow{2}{*}{\makecell{\textit{Avg.}\\\textit{Len.}}}\\ \cmidrule{4-8} 
 &  &  & 1 & 2 & 3 & 4 & 5 &  \\ \midrule
Flow Matching\ \  & \multirow{6}{*}{ABC}  & Chunk & 0.910 & 0.812 & 0.730 & 0.652 & 0.573 & 3.68 \\
Flow Matching\ \  & & First  & 0.793  & 0.586  & 0.442  & 0.351  & 0.273 & 2.45 \\
Flow Matching\ \  & & Ensemble  & 0.838  & 0.710  & 0.614  & 0.545  & 0.437 & 3.14 \\ 
% \midrule
MSE+BCE  & & Chunk  & 0.901 & 0.802 & 0.703 & 0.620 & 0.544 & 3.57 \\
MSE+BCE & & First  & 0.822  & 0.564  & 0.371  & 0.265  & 0.169 & 2.19 \\
MSE+BCE & & Ensemble  & 0.880  & 0.730  & 0.606  & 0.508  & 0.414 & 3.14 \\ 
\midrule
% DDPM (Chunk) & \multirow{9}{*}{ABCD}  &   &   &   &   &  & \\
% DDPM (First) &  &   &   &   &   &  & \\
% DDPM (Ensemble) &  &   &   &   &   &  & \\
Flow Matching\ \  & \multirow{6}{*}{ABCD}  & Chunk  & 0.937 & 0.872 &  0.811 & 0.764 & 0.705 & 4.09 \\
Flow Matching\ \ &  & First  & 0.898  & 0.799 & 0.701 & 0.618 & 0.544 & 3.56 \\
Flow Matching\ \ & & Ensemble &  0.945 & 0.882  & 0.818  & 0.770  & 0.708 & 4.12\\
MSE+BCE  & & Chunk  & 0.933 & 0.863 & 0.808 & 0.751 & 0.688 & 4.04 \\
MSE+BCE & & First  & 0.925 & 0.727 & 0.579 &  0.473 & 0.378 & 3.06 \\
MSE+BCE & & Ensemble  &  0.925 & 0.849 & 0.784  & 0.721  & 0.664 & 3.94 \\ 

\bottomrule
\end{tabularx}
\label{tab:train_loss}
    \end{subtable}
    
    \vspace{0.5cm}
    
    \begin{subtable}{\textwidth}
        \centering
        \caption{Effectiveness of Mix-of-Expert structure}
        \begin{tabularx}{\textwidth}{l@{\extracolsep{\fill}}|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X|>{\centering\arraybackslash}X} 
\toprule
\multirow{2}{*}{\makecell{Training\\Objective}} & \multirow{2}{*}{\makecell{Using\\MoE}} & \multicolumn{5}{c|}{Consecutive tasks success rates} & \multirow{2}{*}{\makecell{\textit{Avg.}\\\textit{Len.}}}\\ \cmidrule{3-7} 
 &  & 1 & 2 & 3 & 4 & 5 &  \\ \midrule
MSE+BCE & \checkmark (ABC) & 0.932 & 0.824 & 0.732 & 0.644 & 0.556 & 3.69   \\
MSE+BCE & \ding{55} (ABC) & 0.901 & 0.802 & 0.703 & 0.620 & 0.544 & 3.57 \\
Flow Matching \ \ & \checkmark (ABC) & 0.940 & 0.855 & 0.768 & 0.679  & 0.597  & 3.84   \\
Flow Matching \ \  & \ding{55} (ABC) & 0.910 & 0.812 & 0.730 & 0.652 & 0.573 & 3.68 \\ 
\midrule
MSE+BCE & \checkmark (ABCD) & 0.945 & 0.823 & 0.678 & 0.561 & 0.457 & 3.46  \\
MSE+BCE & \ding{55} (ABCD) & 0.933 & 0.863 & 0.808 & 0.751 & 0.688 & 4.04 \\
Flow Matching \ \ & \checkmark (ABCD) & 0.911 & 0.828 & 0.759 & 0.707 & 0.639 & 3.84 \\
Flow Matching \ \  & \ding{55} (ABCD) & 0.937 & 0.872 &  0.811 & 0.764 & 0.705 & 4.10 \\

\bottomrule
\end{tabularx}
\label{tab:moe}
    \end{subtable}
\end{table*}

% While for long-horizon tasks like the ones in CALVIN that require the robot to execute five consecutive tasks, introducing history into the policy head could boost the performance for the latter tasks, the success rate for finishing the first task in the sequence has not been significantly improved. This explains the reason that many existing VLAs~\citep{black2024pi_0, kim2024openvla, liu2024robomamba} adapt the \texttt{One-Step-Continuous} architecture, it is training efficient and could achieve comparable performance for single-skill non-compositional tasks, including pick / place, open / close, and etc. 
\red{Yet, the historical formulation is demonstrated to have the best performance, most recent learning-based techniques favor the one-step-continuous formulation for its computational efficiency, with an acceptable performance drop on short-horizon tasks. This offers a practical trade-off, particularly for real-robot deployment~\citep{black2024pi_0, kim2024openvla}. To further investigate their impacts on the performance of resulting policies, we based them on the state-of-the-art one-step-continuous formulation with the best-performing PaliGemma backbone, to align with their original backbone setting and ensure fair comparison.}

\question{3.3}{How do training objectives and inference-time aggregation strategies impact the performance?}

% However, even the \texttt{One-Step-Continuous} VLAs all take the current visual observation as input, their training objectives and executing paradigms are diverse. In this work, we mainly consider three most common training objectives:
\red{Learning-based policies vary in training objectives and inference, leading to different execution behaviors. For example, in behavior cloning, the most prevailing way is to use MSE or BCE losses for action generation, while diffusion policies learn denoising trajectories through generative modeling. We investigate different training objectives along with the widely-exploited inference-time aggregation strategies for a comprehensive understanding.}

In detail, we compare the following two objectives, which are the most prevailing ones in current days:
\begin{itemize}
    % \item {\bf DDPM~\cite{chi2023diffusion, ddpm, ke20243d}}. Add gaussion noise to the action tokens and the model's learning objective is to denoise the action tokens and reconstruct the original action.
    \item \red{{\bf Flow Matching~\cite{lipman2022flow, black2024pi_0}} is a diffusion-based objective. It regards the denoising process as a continuous flow and samples timestep $t\in [0, 1]$ to enforce the model to predict the velocity at $t$. For inference, the model randomly samples an action-chunk shaped gaussion noise, and predicts the denoising velocity based on the current action chunk and time step, the denoised velocity is added to the action chunk vector until the maximum denoising step is reached. }
    \item \red{{\bf MSE+BCE~\cite{wu2023unleashing, li2023vision}}. It formulates the action as an $ n+1$-dimensional vector, with $n$ continuous actions representing arms or end-effector poses, plus a separate gripper action. It utilizes Mean Square Error (MSE) to learn the continuous actions and Binary Cross Entropy (BCE) to learn the state of the gripper.}
\end{itemize}

\red{Besides, we also compare different inference-time action aggregation strategies including \textit{Chunk}, \textit{First}, and \textit{Ensemble}:}
\begin{itemize}
    \item \red{\textbf{Chunk}: A chunk will be fully executed before the next inference.}
    \item \red{\textbf{First}: Only the first action in the chunk will be executed, and then run the next inference.}
    \item \red{\textbf{Ensemble}: An ensemble strategy \cite{zhao2023learning} is used to aggregate the predictions at the same time step from different action chunks.}
\end{itemize}

From Table.~\ref{tab:train_loss} we could observe that:
\begin{itemize}

\item \red{\textbf{Diffusion policies do not significantly improve performance compared to MSE+BCE.} While Flow Matching slightly outperforms MSE+BCE in all experiments, the performance gap is not significant. This suggests that the added inference-time complexity of diffusion models offers limited benefit for short-horizon tasks where deterministic objectives already perform well.}
    
    % \item Diffusion based policies tend to achieve their best performance through executing the action chunk. This is reasonable since the diffusion policies model the trajectories as a multimodal distribution, so that each sampled trajectory could be very different with each other. Only by executing the entire action chunk could obtain a suitable trajectory, executing the first action or ensembling with other overlapped history chunks could destory the action chunk.
    
    % \item For deterministic policies (MSE+BCE), action ensembling achieves the best performance. This is because the mse loss could be viewed as a smoothing among all related trajectories, so that the moving patterns between different action chunks are more consistent. So that ensembling the actions within serval chunks get a more reasonable trajectory with lower variance while maintain the moving pattern of the trajectory.
    
\item \red{\textbf{One-Step-Continuous policies benefit most from executing full action chunks.} Across both Flow Matching and MSE+BCE, the Chunk paradigm consistently yields the best performance in novel scenarios (Training Split ABC). This is likely because the models learn to generate trajectories from a multimodal distribution, and executing only the first action or aggregating across chunks (as in Ensemble) can introduce mode collapse or distort the intended trajectory. Chunk execution preserves temporal coherence within the sampled sequence. While in seen scenarios (Training Split ABCD), executing action chunks does not achieve significant performance improvement compared with ensembling. This indicates that in seen scenarios, the diversity of trajectories might be decreased so that executing action chunks is comparable with ensembling. However, chunking execution could decrease the inference times of VLAs and achieve a real-time deployment (over 30HZ), so that for the rest of the experiments, we utilize chunking execution for one-step-continuous policies.}

\item \red{\textbf{Executing only the first action underperforms across both objectives.} The First paradigm results in significantly lower performance regardless of training objective, especially as the sequential task progresses. This suggests that relying solely on the first action from a sampled or predicted sequence lacks the temporal context and consistency, which are particularly necessary for long-horizon task success.}


\end{itemize}

\finding{3.3}{\red{For \texttt{One-Step-Continuous} formulation, Diffusion loss and MSE loss could achieve a similar performance. For inference-time aggregation strategy, it is important to keep execution consistency, particularly for long-horizon tasks and multimodal actions.}}

% Since the performance of diffusion head and Fully-Connecting (FC) head are similar, we utilize FC head as the default implementation for \texttt{One-Step-Continuous} models. 
% As proposed in \citet{black2024pi_0}, besides leveraging the VLM backbone, an action expert is added into each layer of the VLM. This is motivated by the Mix-of-Expert (MoE) structure proposed in \citet{moe}, which introduces multiple Feed Forward Networks (FFN) into each VLM layer and learns a dyanmic routine for the forward process. To maintain the original vision-language alignment and understanding ability of the VLMs, $\pi_0$ designs a fixed routine in which the original VLM modules (including self-attention and feed forward network) process the vision and language tokens, while the action expert processes the action tokens. 
% Note that the action tokens would interact with the vision and language tokens through the self-attention mechanism to fuse the information.
% While this design is intuitively reasonable, we need to verify whether it could help improve the performance. 
\red{Inspired by the Mixture-of-Experts (MoE) in deep learning \citep{moe}, which dynamically routes inputs through specialized feed-forward networks, $\pi_{0}$ \cite{black2024pi_0} proposes augmenting each VLM layer with a dedicated action expert. This design, used in the $\pi_0$ \cite{black2024pi_0} and $\pi_{0.5}$ \cite{intelligence2025pi_}series, preserves vision-language reasoning by routing vision and language tokens through the original VLM modules, while action tokens are handled by the expert and fused via self-attention. Given its demonstrated effectiveness, we also investigate the impact of this structure under our policy formulation.}
\question{3.4}{Does Mix-of-Expert structure benefit VLA learning?}

% \input{tables/pali_moe}

% To answer this question, we implement the MoE structure with four different formulations: namely, Fully-Connected MSE (FC MSE), Fully-Connected Flow Matching (FC FM), DiT and LSTM.
% As shown in Table.~\ref{tab:moe}, we can get the following observations:
% \begin{itemize}
%     \item TODO: investigate the influence of MoE structure for different policy heads.
% \end{itemize}
\red{To assess the effectiveness of the MoE design, we adopt the same setup as the $\pi$-series as shown in Extended Fig. 2a where the vision-language (VL) tokens are processed by the standard VLM feedforward network (FFN), and the action tokens are routed through a separate action expert FFN. The two sets of tokens interact via self-attention, maintaining joint reasoning while allowing specialization. We evaluate this structure under two representative training objectives: MSE+BCE and Flow Matching, which follow both our default settings in this paper and the original setting in $\pi$-series, respectively.}

% \red{From Table.\ref{tab:moe}, we observe that MoE consistently improves generalization across training objectives. For both MSE+BCE and Flow Matching, using the MoE structure yields higher success rates across all five consecutive tasks in the visually zero-shot setting (Training Split ABC). This suggests that the MoE structure can indeed improve generalization consistently. However, for seen scenarios (ABCD), introducing MoE structure could not benefit the performance, both training objectives achieve higher success rates without MoE structure. This indicates that for scenes that are similar or identity with training scenarios, directly utilizing the original VLA backbone is enough.
From Table.~\ref{tab:moe}, we observe that
\begin{itemize}
    \item \red{MoE structure consistently improves generalization in the visually zero-shot setting (Training Split ABC). For both MSE+BCE and Flow Matching training objectives, using MoE yields higher success rates across all five consecutive tasks. This suggests that MoE enhances the model’s ability to generalize to unseen scenarios. This demonstrates that the mixture-of-experts (MoE) structure is beneficial in preserving the pretrained vision-language (VL) capabilities, as the action prediction does not impose strong supervision on the visual tokens. }

    \item \red{For seen scenarios (Training Split ABCD), introducing the MoE structure does not provide additional benefits. Both training objectives achieve higher success rates without MoE, suggesting that for scenes similar or identical to the training data, the original VLM backbone is sufficient. This may originate from that the MoE structure tends to preserve the general pretrained vision-language (VL) representations, whereas directly fine-tuning the VLA backbone without MoE allows the model to specialize instead of generalize, and fit more effectively to the seen tasks, leading to better performance under familiar settings.}

\end{itemize}

\finding{3.4}{Introducing the Mix-of-Expert structure can improve the generalization of VLAs, while it can not boost the performance in seen scenarios.}

\subsection{When should we leverage the public diverse robot data for optimal training?}

% \begin{figure}[!h]
%   \centering
%   \includegraphics[width=0.7\linewidth]{imgs/cross_emb_setting.jpeg}
%   \caption{
%   % Illustration of the considered traning settings for Bridge and Google Robot. The green tick refers to data that are involved, and the text represents the training stages that utilized the data source. While the red cross illustrates that the data source is not involved in neither training stage. For example, Bridge Post Train consists of two training stages, stage 1 utilizes cross embodiment data, Bridge V2 dataset, RT1 target dataset and RT1 extra data to cotrain the model, and stage 2 further leverage Bridge V2 dataset to post train the model.
%   \textcolor{black}{Illustration of training configurations for Bridge and Google Robot. The red crosses (\ding{55}) denote the excluded training stage, and the small icons represent the datasets used, corresponding to those shown above in the figure. Take Bridge Post Train as an example, two stages are employed: Stage 1: Co-training with cross-embodiment data, Bridge V2 dataset, RT1 target dataset, and RT1 extra data. Stage 2: Post-training refinement using only the Bridge V2 dataset.}
%   % Green checkmarks ($\checkmark$) indicate data sources utilized in training stages, while red crosses (\ding{55}) denote excluded data. Corresponding text labels specify the training stages leveraging each data source.Example: For Bridge Post Train, two stages are employed: Stage 1: Co-training with cross-embodiment data, Bridge V2 dataset, RT1 target dataset, and RT1 extra data. Stage 2: Post-training refinement using only the Bridge V2 dataset.
%   }  
%   \label{fig:cross_setting}  
%   \vspace{-10pt}
% \end{figure}

% \begin{figure}  
%   \centering
%   \includegraphics[width=0.85\linewidth]{imgs/cross_embodiment.pdf}
%   \caption{Ablation studies for cross-embodiment training on \textbf{SimpleEnv}. We evaluate four different training recipes. On the \textit{WidowX+Bridge} environments, we test (1) Bridge \textbf{\textit{Finetune}} finetunes the VLA directly on the full Bridge datasets (tested tasks not included); (2) OXE \textbf{\textit{Co-Train}} Co-trains the VLA on OXE dataset~\citep{o2023open}; (3) \textit{\textbf{Post-Train}} trains the OXE Co-trained VLA on Bridge datasets. 
%   On the \textit{Google Robot} environments, we test (1)
%   \textit{RT-Partial \textbf{Finetune}} finetunes the VLA on tested RT tasks only; (2) \textit{RT \textbf{Finetune}} finetunes the VLA on the full RT dataset (tested tasks included), along with (3) \textit{OXE \textbf{Co-Train}} and (4) \textit{\textbf{Post-Train}} on the tested RT tasks stage.}  
%   \label{fig:cross_emb}  
%   \vspace{-15pt}
% \end{figure}

In recent work, it has been a dominant trend to leverage large-scale cross-embodiment robot manipulation datasets to improve the performance of VLAs~\citep{kim2024openvla, black2024pi_0, brohan2023rt, o2023open}. 
However, it is still not fully clear if it helps and an important question remains:
\question{4}{How do large-scale cross-embodiment datasets contribute to VLAs?}

To address this, we break the question into two sub-questions:
\begin{enumerate}
    \item What types of data from large-scale cross-embodiment datasets are the most beneficial for building VLAs?
    \item When and how should these data be utilized effectively?
\end{enumerate}

\textcolor{black}{In this section, we conduct a series of experiments to investigate different strategies for using external large-scale cross-embodiment datasets. Specifically, we explore three settings as shown in Extended Fig.~\ref{fig:cross_setting}}:
\begin{itemize}
    \item \minghuan{\textit{\textbf{Co-train}}: Training the model with in-domain manipulation data and cross-embodiment datasets. Previous work like RT-2~\citep{brohan2023rt}, OpenVLA~\citep{kim2024openvla}, and OCTO~\citep{team2024octo} only consider this one-stage training.}
    
    \item \minghuan{\textit{\textbf{Post-train}}: First, Co-training the VLMs on in-domain and cross-embodiment datasets as above; then, fine-tuning with in-domain manipulation tasks. This has been adopted by $\pi_0$~\citep{black2024pi_0}.}

    \item \minghuan{\textit{\textbf{Finetune}}: Without involving cross-embodiment datasets, fine-tuning the model with only in-domain manipulation tasks. For RT1 dataset that includes the exact target tasks, we further split the RT1 dataset into target tasks and extra in-domain data.}
\end{itemize}

Our experiments in this section use the best-performing KosMos backbone with a policy head for history fusion as the base model. We use Open X-Embodiment (OXE)~\citep{o2023open} as the cross-embodiment dataset, which comprises a diverse range of robot manipulation data collected worldwide and is the most widely used one in recent works~\citep{brohan2023rt, black2024pi_0, kim2024openvla, team2024octo}.

\noindent\textit{D.1 In Domain Evaluation}

We first test on the general in-domain tasks (i.e., tasks inside OXE).
For comparison, we also evaluate a baseline setting, \textit{\textbf{Finetune}}, where the VLA is trained exclusively on in-domain data. 
Additionally, for \textbf{Google Robot}, we include both \textit{RT-Partial \textbf{Finetune}} and \textit{RT \textbf{Finetune}}, where \textit{RT-Partial \textbf{Finetune}} involves only the trajectories with the same task type as the evaluating tasks, and \textit{RT \textbf{Finetune}} involves co-finetuning the policy with additional data from the same robot across different tasks. For \textit{Bridge}, we only evaluate \textit{Bridge \textbf{Finetune}}, which finetunes the policy with the entire \textit{Bridge-V2} dataset, since the training dataset does not contain trajectories with the same instructions as the evaluated tasks. 


The comparison of the two stages of using cross-embodiment data is shown in Extended Fig.~\ref{fig:cross_emb}, showing the evaluation results for \textbf{SimplerEnv}-\textit{Google Robot} and \textbf{SimplerEnv}-\textit{Bridge}, from which the following observations can be drawn:
\begin{itemize}
    \item \textbf{\textit{Co-training} on cross-embodiment data without post-training does not help significantly.} Comparing \textit{OXE \textbf{Co-train}} and \textit{RT-Partial \textbf{Finetune}} reveals that for both \textit{Google Robot} and \textit{Bridge}, co-training with cross-embodiment data does not lead to substantial performance improvements. In particular, for \textit{Google Robot}, training with additional in-domain data (\textit{RT \textbf{Finetune}}) from different tasks achieves higher success rates (compared with \textit{RT-Partial \textbf{Finetune}}). This indicates that in-domain data, even if task-agnostic, is more effective for improving model performance than cross-embodiment data.

    % \item \textbf{\textit{Post-training} after cross-embodiment pre-training shows potential benefits.} The average performance of the post-trained model (52\% on \textit{Google Robot} and 38\% on \textit{Bridge}) exceeds that of the model fine-tuned exclusively on in-domain data (48\% on \textit{Google Robot} and 31\% on \textit{Bridge}). This suggests that cross-embodiment pre-training can provide a useful initialization that benefits subsequent fine-tuning.

    \item \red{\textbf{\textit{Post-training} shows potential benefits over high-frequency tasks in the first co-training stage.} The average performance of the post-trained model exceeds that of the model fine-tuned exclusively on in-domain data on \textit{Bridge} (50\% for post-trained and 44\% for fine-tuned). While for \textit{Google Robot}, the post-trained model only outperforms the fine-tuned model over \texttt{pick coke can} tasks, and drops its performance on all other tasks. We consider the main reason is that the proportion of \texttt{pick-and-place}tasks in the OpenX-Embodiment dataset is very large, so that the post-trained model gains higher performance over \texttt{pick-and-place} tasks, while it loses performance over tasks involving other skills like \texttt{move near} and \texttt{open/close drawer} as a trade-off. 
    In other words, cross-embodiment co-training enables VLAs to learn skills for high-frequency tasks from other types of embodiments and transfer the acquired knowledge to the target embodiment during the post-training phase. This helps VLAs further improve the overall success rate of these tasks, though at the cost of sacrificing low-frequency tasks and skills in the co-training stage.}
    % This suggests that cross-embodiment pre-training can provide a useful initialization that benefits subsequent fine-tuning.

    \item \red{\textbf{In-domain data plays a critical role in achieving strong task performance.} Even task-agnostic in-domain data from the same embodiment (e.g., RT Finetune) proves more effective than large-scale cross-embodiment data for fine-tuning VLAs, as shown by the experiments on \textit{Google Robot} dataset, especially for fitting specific tasks. While cross-embodiment pre-training can provide useful initialization in some cases, leveraging in-domain data remains essential for robust and consistent policy performance.}
    
\end{itemize}

\noindent\textit{D.2 Out-of-Distribution Evaluation}

To evaluate the impact of cross-embodiment datasets more comprehensively, we further perform experiments on \textbf{CALVIN}, whose data is not part of OXE. We mainly focus on whether cross-embodiment datasets benefit \textit{\textbf{few-shot learning}} (we randomly sample 10 trajectories for each task from data split ABCD for training and test on D) on out-of-distribution tasks (w.r.t. to OXE). To keep settings consistent, we only take the image from the static on-head camera as input. The results are illustrated in Extended Fig.~\ref{fig:few_shot}, and we conclude that: 

\begin{itemize}
    \item \textbf{Cross-embodiment \textit{pre-training} improves \textit{few-shot learning} performance.} In the few-shot setting for CALVIN, with a single-view on-head camera, pre-training significantly improves the performance by 17.2\% in terms of single-task execution and 0.25 more executed tasks in each rollout.
    It can be concluded that pre-training on large-scale cross-embodiment datasets benefits the learning of more effective representations for robot manipulation, which can quickly adapt to novel manipulation tasks with unseen objects and environmental settings.
\end{itemize}

\finding{4}{Extra in-domain data, even from different tasks, shows beneficial, and an extra large-scale cross-embodiment co-training before the post-training stage further improves high-frequency tasks as well as few-shot performance.}


==> papers/3-conclusions.tex <==
\section{Discussion}\label{sec:discuss}

This empirical study mainly focuses on what matters in building Visual-Language-Action models (VLAs).
We raise four essential questions for building a VLA: {\bf Why} do we need VLAs instead of other generalist policies, and by outperforming the existing methods by a large margin, we illustrate the necessity of studying VLAs. For the next step, we describe the key components for building a VLM-based VLA: {\bf Which} kind of VLM backbone to utilize, {\bf How} to train the model to generate action, and {\bf When} should we add cross-embodiment data into training stages. To answer these questions, we built a unified framework for a fair comparison of VLAs and designed a series of bottom-up systematic experiments. To answer these questions, we conduct extensive experiments across three simulators and more than 240 rollouts within 20 tasks in real-world scenarios, and we can conclude from the experiments that: For the {\bf Why} question, VLAs could achieve high performance and generalization, and is a promising path to generalist robotics policy; For the {\bf Which} problem, we find that VLMs with sufficient vision-language pre-training over large scale vision-language datasets is suitable for constructing VLAs.
For the {\bf How} problem, we can investigate the performance, generalization, and data efficiency of different VLA structures, and find that integrating history observations is essential for VLAs, and policy head is a more effective and efficient history aggregating method compared with interleaved; For the {\bf When} problem, we compare three training recipes with cross-embodiment integrated at different stages, and conclude that extra in-domain data shows beneficial, and large-scale cross-embodiment pre-training further improves overall as well as few-shot performance. As a byproduct of answers to the raised questions, we built an easy-to-use framework for easily integrating arbitrary VLMs and turning them into VLAs, named {\bf RoboVLMs}. 

\noindent\textbf{Under investigated observations.}
During our experiments, we found that VLAs built upon Qwen-VL and LLaVA, the performance is surprisingly low, compared with their original performance on vision-language tasks. After adding a perceiver resampler after the vision encoder, we found that the VLAs based on Qwen-VL and LLaVA could obtain great performance gains and reach reasonable performance. We hypothesize that the performance gain is related to the image resolution and the number of vision tokens in the input token sequence.

\noindent\textbf{Limitations.}
Although we make every effort to investigate the key challenges in building Vision-Language Agents (VLAs), this work remains preliminary and has several limitations at the current stage.
% (1) For the sake of quick and simple expansion over existing Vision-Language Models (VLMs), we retain the multi-modal interaction structure within the VLM (\textit{e.g.}, attention masks, mixture of experts). On top of this, we further develop the interaction between vision, language, and actions, which is a common approach in most existing works~\citep{kim2024openvla,li2023vision}. However, a specialized design for the architecture and multi-modal interaction with actions has the potential to yield superior performance (e.g., the $\pi_0$ model~\citep{black2024pi_0}), and warrants further exploration.
% (2) The categorizations and formulations of VLAs considered here are simplified and limited for the reasons outlined in (1). 
% Additionally, we have not yet investigated how a mixture of experts (MoE) model~\citep{moe, black2024pi_0} could be integrated into VLAs, nor have we explored how the taxonomy might evolve when such a module is included.
% (3) The action tokenization, policy head, and corresponding training objectives are not fully explored in this work. For example, techniques like VQ-VAE~\citep{van2017neural}, diffusion models~\citep{ddpm, chi2023diffusion}, and flow matching~\citep{lipman2022flow, esser2024scaling, black2024pi_0} remain under-explored in the context of VLAs.
% (4) The set of VLM backbones considered in this study is limited and can be actively expanded.
% (5) Deploying such large models for real-time robotic control remains a significant challenge.
(1) The action tokenization, policy head, and corresponding training objectives are not fully explored in this work. For example, techniques like VQ-VAE~\citep{van2017neural}, VQGAN~\citep{esser2021taming}, and FAST action tokenizer~\citep{pertsch2025fast} remain under-explored in the context of VLAs.
(2) The set of VLM backbones considered in this study is limited and can be actively expanded.
(3) Deploying such large models for real-time robotic control remains a significant challenge.

\noindent\textbf{Future works.} For future work, we envision several potential directions for advancing generalist robot policies. 
% 1) As aforementioned, our current approach faces limitations in the design of internal structures for VLMs, policy heads, and corresponding training objectives. Further investigation into more fine-grained design choices for VLAs could be highly valuable, as recent studies suggest they play a significant role in improving efficiency and effectiveness~\citep{black2024pi_0}. 
Beyond semantic generalization, an ideal generalist robot policy should be capable of handling long-horizon, complex task instructions (e.g., \texttt{make breakfast}), reasoning through executable actions step by step, and generating meaningful physical interactions with its environment (e.g., \citep{zawalski2024robotic}). In our future work, we aim to explore the key elements required to develop policies with these advanced capabilities.

We have open-sourced our codebase with detailed guidelines, model weights of the strongest VLAs built by RoboVLMs, along with the real-world dataset used in our experiments. 
We anticipate that our research will bolster the community and expedite progress in the realms of vision-language learning and foundational models for robotics.


==> papers/4-method.tex <==
\section{Method and Material}
\label{sec:method}

We consider the problem of controlling a robot to accomplish a set of tasks, based on language instructions $l$, and historical observations $o_{t-H+1:t}$ at every time step $t$ with the maximum historical length $H$.
In this paper, we mainly consider a table-top robot arm, therefore the observations $o_t$ are sensor inputs and images, e.g., $o_t = (s_t, I_t)$, from either a third-view camera, a gripper camera, or both.
We build a controlling policy $\pi(a|o_{t-H+1:t},l)$, where the action $a$ is modeled as a 7-dim vector, including the 6-DoF pose of the gripper, along with its open/close status. 
In this section, we will first introduce the formulation of vision-language models (Section \ref{sec:vlm}), based on which we build our VLA formulations.

\subsection{Vision Language Model}
\label{sec:vlm}
Vision-language models (VLMs), also referred to as multi-modal large language models, integrate vision into their input modality, enabling them to process and reason about both visual and textual information. Typically, VLMs are prompted with images and/or text to generate text~\citep{liu2024visual, bai2023qwen, alayrac2022flamingo, moondream, uform-gen, beyer2024paligemma}, facilitating applications such as image captioning, visual question answering, and goal-directed planning. 
This process can be formally described as:
\begin{equation}
    \hat{l} = \text{VLM}(I, l_{\text{prompt}})~.
\end{equation}
Here, $I$ and $l_{\text{prompt}}$ denote the image and text prompts, respectively, while $\hat{l}$ represents the text output generated by the VLM. For instance, in a visual question-answering task, $l_{\text{prompt}}$ corresponds to the question, and $l_{\text{target}}$ corresponds to the generated answer.
Training a VLM typically involves minimizing a cross-entropy loss to predict discrete language tokens, which can be expressed as:
\begin{equation}
    \ell_{\text{VLM}} = \text{CrossEntropy}(\hat{l}, l_{\text{target}})~,
\end{equation}
where $l_{\text{target}}$ is the ground truth text.
By pre-training on millions or even billions of paired vision-language data, VLMs acquire robust representations of both visual and textual modalities.
To effectively handle these two distinct modalities, VLMs typically employ a vision processor and a language decoder, connected through various vision-language feature fusion mechanisms. Among the available options, vision transformer (ViTs)~\citep{dosovitskiy2020image} and perceiver resampler~\citep{jaegle2021perceiver} are widely adopted choices for the vision processor~\citep{li2023vision, team2024octo, liu2024robomamba, wu2023unleashing}. The ViT module reshapes each input image $I$ into patches and encodes them as visual tokens \texttt{[OBS]}:
\begin{equation}
    \texttt{[OBS]} = (x^v_1, \cdots, x^v_N) = \text{ViT}(I)~,
\end{equation}
where $N$ represents the token number, $x^v_i$ represents the $i$th token, which, in ViT, is an embedding vector encoding a patch of the input image. 


Existing VLMs can be broadly categorized into two structural paradigms: encoder-decoder and decoder-only architectures. These two structures differ mainly in their multi-modal fusion strategies.

{\noindent\bf Encoder-decoder}. Encoder-decoder architectures are composed of two main components: 
an encoder that is typically responsible for extracting features from inputs using input embedding modules as discussed above, and a decoder that generates the output (e.g., text or multi-modal predictions) auto-regressive. 
Feature fusion between the encoder and decoder is usually achieved by cross-attention layers in the decoder. 
This structure excels in tasks requiring a detailed understanding of the input modalities, such as image captioning and visual reasoning, due to its ability to explicitly encode multi-modal information prior to generation~\citep{nagrani2021attention, xu2021vlm}. Representative models include Flamingo~\citep{alayrac2022flamingo} and OFA~\citep{wang2022ofa}.

{\noindent\bf Decoder-only}. Decoder-only architectures, in contrast, rely on a unified transformer framework where both the input modalities (vision and text) and the output sequences are processed in the same autoregressive decoder. In these models, visual features are first embedded into token-like representations (via vision processors), which are then concatenated with textual tokens and passed through the decoder. 
Multi-modal feature fusion occurs naturally through the self-attention mechanism, allowing the decoder to model dependencies between visual and textual inputs during token generation. Decoder-only architectures are more flexible and scalable, making them well-suited for tasks like instruction following, multi-modal question answering, and open-ended generation. Examples of decoder-only models include GPT-4V~\citep{yang2023dawn} and LLaVA~\citep{liu2024visual}.

\subsection{Vision-Language-Action Models}
\label{sec:vla}

% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=.95\textwidth]{imgs/framework_v2.pdf}
%     \caption{The illustration of considered VLA formulations, including several popular designs. For example, RoboFlamingo~\citep{li2023vision} is a \texttt{Policy-Head-Continuous}-type VLA, RT-2~\citep{brohan2023rt} and OpenVLA~\citep{kim2024openvla} corresponds to the \texttt{One-Step-Discrete-Action}-type VLA. Octo~\citep{team2024octo} and GR~\citep{wu2023unleashing} correspond to the \texttt{Interleaved-Continuous-Action}-type VLA with a fixed window size.}
%     \label{fig:framework}
% \end{figure*}

Vision-language-action models (VLAs) are predominantly applied to robotic tasks, where they serve as a generalist robot policy $\pi$ capable of handling complicated tasks. In formal, VLAs predict action sequences based on previous observations at the current time step $t$:
\begin{equation}\label{eq:vla-general}
    a_{t:t+L-1} = \text{VLA}(o_{t-H+1:t}, l_{\text{prompt}})~,
\end{equation}
where $a_{t:t+L-1}$ are a sequence of predicted 7-dim actions, $L$ is the action sequence length and $H$ is the history observation length.
Different from VLMs, the observations of VLAs $o_{t-H+1:t}$ usually contain proprioceptive states $s_{t-H+1:t}$ like the joint angles and end-effector positions besides the visual inputs $I_{t-H+1:t}$.
As discussed in Section \ref{sec:vla}, we abstract and categorize VLAs into four representative structures based on 1) historical information modeling and 2) action space. Before we describe these distinct models in form, we first introduce the general pre-process and prediction principles when dealing with robot actions in different action spaces.

\noindent\textit{1) Action Pre-process}

\noindent\textbf{Action Normalization.}
For both continuous and discrete action spaces, we normalize each dimension of the 7-DoF action. Following \citet{kim2024openvla}, we count the 1\textsuperscript{st} and 99\textsuperscript{th} quantile of the actions in the training data and use the quantiles to clamp each dimension of the action~\citep{brohan2023rt}:
\begin{equation}
    a^{i'} = \min(a^i_{ 99\textsuperscript{th}}, \max(a^i_{1\textsuperscript{st}}, a^i))~,
\end{equation}
where $a^{i'}$ is the clamped value of the $i$-th dimension of action $a$. For the next step, we normalize each dimension of the clamped action $a^{'}$ with the 1\textsuperscript{st} and 99\textsuperscript{th} quantile of the actions:
\begin{equation}
    \Tilde{a}^i = 2 \times (a^{i'} - a^i_{1\textsuperscript{st}}) / (a^i_{ 99\textsuperscript{th}} - a^i_{1\textsuperscript{st}}) - 1~.
\end{equation}
$\Tilde{a} = [\Tilde{a}^1, \Tilde{a}^2,\cdots, \Tilde{a}^7]$ is the normalized action, each dimension is in the range of $[-1, 1]$, the last dimension representing the open/close status of the gripper $\in \{-1, 1\}$.
During inference time, we will reversely map the predicted actions into unnormalized actions.

\noindent\textbf{Action Discretization.}
For discrete action representation, we need to further discretize the normalized action $\Tilde{a}$. Following \citet{brohan2023rt, kim2024openvla}, we map continuous robot actions to discrete tokens used by the VLM's tokenizer. Specifically, we discretize each robot action dimension into one of 256 bins separately. For each dimension, we set the width of the bin to uniformly divide the interval between the quantile of 1\textsuperscript{st} and 99\textsuperscript{th} of actions in the training data.

Using this discretization, we transform $\Tilde{a}$ to $\overline{a}$ with 7~discrete integers $\in [0 \dots 255]$. To avoid damaging the original special token positions in the language tokenizer, we add an offset (default set to 10) and replace the last offset $\sim$ 256+offset tokens with a discretized index.

\noindent\textit{2) Action Prediction}
\noindent{\bf Continuous Actions.}
We optimize the mean square error (MSE) and binary cross entropy (BCE) for the predicted action sequence $a_{t:t+L-1}$ with the ground truth action sequence $\Tilde{a}_{t:t+L-1}$:
\begin{equation}
    l_{\text{VLA}} = \sum_{i=t}^{t+L-1} \text{MSE}(\hat{a}_{i,pose}, \Tilde{a}_{i, pose}) + \lambda * \text{BCE}(a_{i, gripper}, \Tilde{a}_{i, gripper})~,
\end{equation}
where the MSE loss is computed for the first six dimensions, and the BCE loss is for the last gripper dimension between the predicted action $\hat{a}_{t:t+L-1}$ and the ground truth $\Tilde{a}_{t:t+L-1}$, $\lambda$ is the balancing weight. 

\noindent{\bf Discrete Actions.}
Discrete-action models predict action tokens $\texttt{ACT}^i$ for each action dimension $i$.
These tokens are the index of discretized bins from continuous action by dimension, which can be easily de-tokenized to recover the action vector.
The optimization object has a similar cross-entropy (CE) format as text generation widely used in VLM training:
\begin{equation}
    l_{\text{VLA}} = \sum_{i=t}^{t+L-1} \sum_{j=1}^7 \text{CE}(\texttt{[ACT]}^{j}_{i}, \tilde{a}^j_i)~,
\end{equation}
where $\texttt{[ACT]}^{j}_{i}$ represents the index of bins of the $j$$\textsuperscript{th}$ dimension of the predicted action token $\texttt{[ACT]}$ at time $i$, and $\overline{a}^j_i$ is the corresponding ground truth.
During inference time, after getting the predicted action token $\texttt{ACT}^i$, we re-project the discrete tokens to the center of the corresponding bins into a continuous form for achieving tasks.

\subsection{VLA Structures}
As shown in Extended Fig. 3b, there are mainly four kinds of VLA structures categorized by action space and history aggregating method, namely one-step-continuous-action models, one-step-discrete-action models, interleaved-continuous-action models, and policy-head-continuous-action models. Note that our proposed framework RoboVLMs could transfer VLMs to arbitrary VLA structures with no effort. We will illustrate the four VLA structures in detail in the following section.
\noindent\textit{1) One-step Models}
One-step models predict future action sequences using only the observation at the current time step $t$, i.e., a history length of 1.
\begin{equation}\label{eq:vla-onestep}
    \hat{a}_{t:t+L-1} = \text{VLA}(o_{t}, l_{\text{prompt}})~.
\end{equation}
For one-step models, we formulate two variants: {continuous-action model} and {discrete-action model}:

\noindent \textbf{Continuous-action model}: In the continuous-action formulation, the VLM model first predicts a learnable token \texttt{[LRN]} using the VLM backbone. This is achieved by fusing visual and language tokens (in an encoder-decoder architecture) or concatenating multi-modal tokens (in a decoder-only architecture). An MLP is then used to predict the action vector:
\begin{equation}\label{eq:vla-onestep-cont}
\begin{aligned}
    \texttt{[LRN]} &= \text{VLM}(o_{t}, l_{\text{prompt}})~,\\
    \hat{a}_{t:t+L-1} &= \text{MLP}(\texttt{[LRN]})~.
\end{aligned}
\end{equation}
The one-step continuous-action models include ACT~\citep{zhao2023learning}, BC-Z~\citep{jang2022bc}, MVP~\citep{radosavovic2023real}, R3M~\citep{nair2022r3m}, VIMA~\citep{jiang2022vima}, 3D Diffuser~\citep{ke20243d}, RoboMamba~\citep{liu2024robomamba}, and $\pi_0$~\citep{black2024pi_0}.

\noindent \textbf{Discrete-action model}: For discrete action prediction, we directly follow the straightforward next-word prediction similar to VLMs, where actions are discretized into tokens like texts:
\begin{equation}\label{eq:vla-onestep-disc}
\begin{aligned}
    \texttt{[ACT]}^{1:7}_{t:t+L-1} &= \text{VLM}(o_{t}, l_{\text{prompt}})~.
\end{aligned}
\end{equation}
The one-step discrete-action models include RT-1~\citep{brohan2022rt}, RT-2~\citep{brohan2023rt}, 3D-VLA~\citep{zhen20243d}, LAPA~\citep{ye2024latent}, OpenVLA~\citep{kim2024openvla}, and Embodied-COT~\citep{zawalski2024robotic}.

\noindent\textit{2) Interleaved-Continuous-Action Models}
Interleaved models receive observation-action sequences:
\begin{equation}
    O_t = (\texttt{[OBS]}_{t-H+1}, \texttt{[LRN]}), ..., (\texttt{[OBS]}_{t}, \texttt{[LRN]})~,
\end{equation}
% $$O_t = (\texttt{[OBS]}_{t-H+1}, \texttt{[LRN]}), ..., (\texttt{[OBS]}_{t}, \texttt{[LRN]})~,$$
where $O_t$ represents the input token sequence at time instant $t$, $\texttt{[OBS]}$ denotes observation tokens and $\texttt{[LRN]}$ denotes the learnable action token and is  duplicated for $H$ times and insert into $O_t$ with an interleaved format. The VLM backbone fuses this sequence (in a decoder-only structure) and predicts the action sequence through an MLP based on each action token:
\begin{equation}\label{eq:vla-interleaved}
\begin{aligned}
    \texttt{[LRN]}_{t-H+1:t} &= \text{VLM}(O_t)~,\\
    \hat{a}_{t:t+L-1} &= \text{MLP}(\texttt{[LRN]}_{t})~.
\end{aligned}
\end{equation}
The $\texttt{[LRN]}_{t}$ which is utilized to predict the action chunk  $\hat{a}_{t:t+L-1}$, represents the $\texttt{[LRN]}$ inserted after $\texttt{[OBS]}_{t}$ and fused with the observations before $t$.
The loss and action unnormalization procedure is identical with one-step continuous action models. At time instant $t$ of inference, the input sequence contains only the current observation $\texttt{[OBS]}_{t}$ and the language instruction $l_{prompt}$, we add the learnable token $\texttt{[ACT]}$ at the end of the input sequence and pass the sequence to the VLM to predict the action. After the robot executes the predicted action, we add the new observation $\texttt{[OBS]}_{t+1}$ and language instruction $l_{prompt}$ to the input sequence to predict the action in the current step.
The interleaved-continuous-action models include GR-1~\citep{wu2023unleashing}, OCTO~\citep{team2024octo}, GR-2~\citep{cheang2024gr}. Note that the interleaved-discrete-action models like GATO~\citep{reed2022generalist} and RoboCat~\citep{bousmalis2023robocat} are out of consideration. 

\subsubsection{Policy-Head-Continuous-Action Models}
Unlike interleaved models, which fuse historical information within the VLM backbone, policy-head VLAs only require the VLM to provide single-step multi-modal representations at each time step $t$:
\begin{equation}\label{eq:policy_head_obs}
\begin{aligned}
    o_t &= (\texttt{[OBS]}_t, \texttt{[LRN]})~, \\
    \texttt{[LRN]}_t &= \text{VLM}(o_{t}, l_{\text{prompt}})~.
\end{aligned}
\end{equation}
Historical information is then modeled and actions are predicted through an additional policy head $h$, such as an RNN~\citep{medsker2001recurrent, chung2014empirical, graves2012long}, transformer~\citep{vaswani2017attention, floridi2020gpt}, or diffusion model~\citep{chi2023diffusion}:
\begin{equation}\label{eq:vla-policy-head}
\begin{aligned}
     a_{t:t+L-1} &= \text{h}(\texttt{[LRN]}_{t-H+1}, ..., \texttt{[LRN]}_{t})~.
\end{aligned}
\end{equation}
The action chunk $a_{t:t+L-1}$ with sequence length $L$ is predicted based on learnable tokens $\texttt{[LRN]}_{t-H+1}, ..., \texttt{[LRN]}_{t}$.
Each of $\texttt{[LRN]}_{t}$ is identical.
Note that the interleaved-continuous-action model is only available for decoder-only backbones.
The policy-head-continuous-action model can be built based on VLM backbones with both encoder-decoder and decoder-only structures.
The main difference comes from the language decoder. The input sequence of the encoder-decoder VLM fuses only contains the text and learnable action tokens, it fuses the multi-modal input with cross-attention where the text tokens combined with the learnable tokens are the keys and values, and vision tokens are the queries. The decoder-only backbone directly concatenates the vision, language, and learnable tokens as input and utilizes self-attention to fuse the multi-modal features. The policy-head-continuous-action models include RoboFlamingo~\citep{li2023vision}, RoboUniview~\citep{liu2024robouniview}, and DeeRVLA~\citep{yue2024deer}.

At every inference step $t$, the current observation $\texttt{[OBS]}_{t}$ and language instruction $l_{\text{prompt}}$ along with a learnable token $\texttt{[LRN]}$ is concatenated as a complete input sequence, which is further passed into the VLM backbone. After the policy head takes $\texttt{[LRN]}$ and predicts the current action sequences, the robot steps with the predicted actions and obtains the new observation for the next round of prediction. 

\subsection{Real Robot Platform}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{imgs/robot_demo.pdf}
%     \caption{The demonstration of our real robot platform. The platform is equipped with a side camera and a wrist camera. }
%     \label{fig:real_robot}
% \end{figure}
As shown in Fig.~\ref{fig:real_robot}, our real robot platform consists of a Kinova Gen-3 robot arm, equipped with a Robotiq 2F-85 parallel-jaw gripper and two cameras: one static camera for capturing the workspace and another camera mounted on the end-effector. The static camera is a Kinect Azure, while the wrist-mounted camera is a RealSense D435i. The workspace is a 55 cm x 24 cm table, and there are more than 40 objects distributed across the evaluated scenes.

As described in Section II, we define one simple setting and four unseen settings for evaluation on this platform. For the convenience of readers, we provide a more detailed introduction to these settings here. In the \textit{Simple} setting, the scene is designed to closely resemble those in the training data. This setting is used to assess the model's ability to fit the training distribution. In the \textit{Unseen Distractors} setting, previously unseen distractor objects are introduced into the scene, but the manipulated objects are still part of the training data. The \textit{Unseen Backgrounds} setting changes the background by adding two new tablecloths that were not present in the training data. One tablecloth differs in color from the white background, while the other features entirely different patterns. In the \textit{Unseen Objects} setting, the robot is tasked with manipulating objects that were not included in the training dataset. The unseen objects used in this setting are the same as those in the Unseen Distractors setting. Finally, in the \textit{Novel Skill Description} setting, we use GPT-4 to generate three unseen synonyms for the verbs in the instructions and randomly select one to replace the original verb, creating a novel skill description. For instance, "press" may be replaced with "hit," "pick up" with "take," "close" with "shut," "pour" with "sprinkle," and so on.

\subsection{Discussions about Structures}
Although we have discussed four representative VLA structures, by a two-level categorization of historical information and action space, readers may notice that these two dimensions are not entirely orthogonal, and not all combinations are discussed and implemented in this work. This is due to architectural limitations and implementation challenges.
For instance, interleaved and policy-head models with discrete action spaces have not been implemented so far, because interleaved models are typically combined with action chunk prediction, where the default lower triangular attention mask cannot effectively mask subsequent actions for later steps.

\section{Data availability}
Datasets used in this study could be found at \url{https://github.com/mees/calvin} (CALVIN), \url{https://github.com/google-deepmind/open_x_embodiment} (Open X-Embodiment), and \url{https://huggingface.co/datasets/robovlms/bytedance_robot_benchmark_20} (BDRBench20).

\section{Code availability}
The source code of this study could be found at \url{https://github.com/Robot-VLAs/RoboVLMs}.

\section{Acknowledgments}
This work was supported in part by the National Natural Science Fund under Grant 62025304 and in part by the National Natural Science Fund for Key International Collaboration under Grant 62120106005. We thank all the members of the robotics research team at ByteDance Research for their assistance in real-world data collection, setup design, robot maintenance, and experiments. The author Minghuan Liu is supported by the ByteDance Scholarship. We also want to thank @YouJiacheng for his active and instructive discussion on X.

\section{Contributions}

\noindent{\textbf{Project Leads}}: Huaping Liu, Xinghang Li, Hanbo Zhang, Minghuan Liu

\noindent{\textbf{Methodology and Codebase}}: Xinghang Li

\noindent{\textbf{Model Training and Evaluation (experimental design, implementation)}}: Xinghang Li, Long Qian, Hanbo Zhang, Dong Wang, Minghuan Liu, Xiao Ma, Jirong Liu


\noindent{\textbf{Real-Robot Deployment \& Experiments}}: Xinghang Li, Peiyan Li

\noindent{\textbf{Paper (logic, figures, visualizations, writing)}}: Xinghang Li, Minghuan Liu, Hanbo Zhang, Long Qian, Bingyi Kang, Xiao Ma, Peiyan Li, Jirong Liu, Di Guo, Huaping Liu, Tao Kong


\noindent{\textbf{Advising}}: Huaping Liu, Tao Kong, Hanbo Zhang, Xiao Ma, Bingyi Kang, Di Guo, Xinlong Wang

\newpage

\begin{extendedfigure*}[t]
  \centering
  % 上面的子图
  \begin{subfigure}[b]{1.0\textwidth}
    \includegraphics[width=1.0\textwidth]{imgs/real_correction_1.jpeg}
    % \caption{}
    \label{fig:real_correction_sub1}
  \end{subfigure}
  % \vspace{-4mm} % 手动调整为负值
  \\[-3mm] % 调整为合适的负间距
  % 中间的子图
  \begin{subfigure}[b]{1.0\textwidth}
    \includegraphics[width=1.0\textwidth]{imgs/real_correction_2.jpeg}
    % \caption{}
    \label{fig:real_correction_sub2}
  \end{subfigure}
  \caption{Visualization for rollouts that the best setting VLA built by RoboVLMs emerges the ability of self-correction. For instance, in the \texttt{Open The Oven} task, the robot\'s first attempt does not reach the oven handle, and it adjusts the end-effector position to re-locate the handle at the second attempt. Note that the training dataset does not contain this kind of data.}
  \label{fig:real_correction}
\end{extendedfigure*}

\begin{extendedfigure}  
  \centering
  \begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=0.95\linewidth]{imgs/moe_demo.pdf}
  \caption{Illustration of Mix-of-Expert structure. In original VLAs, both vision-language tokens and action tokens share the same weights of the original VLM FFN (Feed Forward Network). For the Mix-of-Expert structure, vision-Language tokens and action tokens have separate query, key and value projection layers for self-attention, and have separate feed-forward networks. Action tokens would only interact with vision-language tokens through self-attention. This Mix-of-Expert structure preserves the original parameters and forward process of the VLMs, and is claimed to benefit the generalization for the built VLAs.}  
  \label{fig:moe_structure}  
  \end{subfigure}
  \vspace{0.5cm}

  \begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=0.95\textwidth]{imgs/framework_v2.pdf}
    \caption{The illustration of considered VLA formulations, including several popular designs. For example, RoboFlamingo~\citep{li2023vision} is a \texttt{Policy-Head-Continuous}-type VLA, RT-2~\citep{brohan2023rt} and OpenVLA~\citep{kim2024openvla} corresponds to the \texttt{One-Step-Discrete-Action}-type VLA. Octo~\citep{team2024octo} and GR~\citep{wu2023unleashing} correspond to the \texttt{Interleaved-Continuous-Action}-type VLA with a fixed window size.}
    \label{fig:framework}
  \end{subfigure}
  \caption{The architectures of MoE and considered VLAs.}
\end{extendedfigure}

\begin{extendedfigure}[htbp]
    \centering
\includegraphics[width=0.8\textwidth]{imgs/cross_emb_setting.jpeg}
    \caption{Illustration of training configurations for Bridge and Google Robot. The red crosses (\ding{55}) denote the excluded training stage, and the small icons represent the datasets used, corresponding to those shown above in the figure. Take Bridge Post Train as an example, two stages are employed: Stage 1: Co-training with cross-embodiment data, Bridge V2 dataset, RT1 target dataset, and RT1 extra data. Stage 2: Post-training refinement using only the Bridge V2 dataset.}
    \label{fig:cross_setting}
\end{extendedfigure}

\begin{extendedfigure}  
  \centering
  \includegraphics[width=0.85\linewidth]{imgs/cross_embodiment.pdf}
  \caption{Ablation studies for cross-embodiment training on \textbf{SimpleEnv}. We evaluate four different training recipes. On the \textit{WidowX+Bridge} environments, we test (1) Bridge \textbf{\textit{Finetune}} finetunes the VLA directly on the full Bridge datasets (tested tasks not included); (2) OXE \textbf{\textit{Co-Train}} Co-trains the VLA on OXE dataset~\citep{o2023open}; (3) \textit{\textbf{Post-Train}} trains the OXE Co-trained VLA on Bridge datasets. 
  On the \textit{Google Robot} environments, we test (1)
  \textit{RT-Partial \textbf{Finetune}} finetunes the VLA on tested RT tasks only; (2) \textit{RT \textbf{Finetune}} finetunes the VLA on the full RT dataset (tested tasks included), along with (3) \textit{OXE \textbf{Co-Train}} and (4) \textit{\textbf{Post-Train}} on the tested RT tasks stage.}  
  \label{fig:cross_emb}  
  \vspace{-15pt}
\end{extendedfigure}

\begin{extendedfigure}[htbp]
  \centering
\includegraphics[width=0.4\textwidth]{imgs/calvin_few_shot.pdf}
  \caption{The effect of cross-embodiment pre-training on OXE datasets for \textit{\textbf{few-shot learning}}.}
  \label{fig:few_shot}
\end{extendedfigure}


\begin{extendedtable*}
\caption{The essential questions, research questions, and findings of the study.
}

\centering
\begin{tabular}
{m{0.25\textwidth}m{0.33\textwidth}m{0.35\textwidth}}
\textbf{Essential Questions} & \textbf{Research Questions} & \textbf{Research Findings} \\
\toprule
\multirow{4}{*}{\textit{Q1}: Why \textbf{VLAs}} & \textit{Q1.1}: Are \textcolor{red}{VLAs} a \textcolor{red}{proper choice} for building generalist robot policies? & \textit{A1.1}: VLA is a \textcolor{red}{promising path} towards generalist robot policies. \\
& \textit{Q1.2}: How does the best VLA built with RoboVLMs perform in real-world scenarios? & \textit{A1.2}: The best setup VLA built with \textcolor{red}{RoboVLMs} appears strong \textcolor{red}{effectiveness} and \textcolor{red}{robustness} in \textcolor{red}{real-world} scenarios. \\
\midrule
\multirow{1}{*}{\textit{Q2}: Which \textbf{Backbone}} & \textit{Q2}: Which type of \textcolor{red}{VLMs} are more suitable for constructing VLAs? & \textit{A2}: \textcolor{red}{Sufficient} vision-language pre-trained on \textcolor{red}{large} vision-language datasets benefit VLAs \\ \midrule
\multirow{8}{*}{\textit{Q3}: How to \textbf{Formulate}}
& \multirow{1}{*}{\textit{Q3.1}}: How to select the best-performing VLA \textcolor{red}{structure}? & \textit{A3.1}: \textcolor{red}{Continuous} action space with \textcolor{red}{policy head} to integrate history is the best structure.\\ 
& \textit{Q3.2}: How do different formulations affect the \red{generalization} and \red{data efficiency} for VLAs? & \textit{A3.2}: Leveraging \red{policy head} for history fusion is the best in terms of generalization and data efficiency. \\
& \textit{Q3.3}: How to design appropriate \textcolor{red}{training objective} and \textcolor{red}{execution paradigm}? & \textit{A3.3}: \textcolor{red}{Diffusion} and \textcolor{red}{MSE} training loss are comparable, executing \textcolor{red}{action chunk} is efficient and effective. \\
& \textit{Q3.4}: Does \red{Mix-of-Expert} structure benefit VLA learning? & \textit{A3.4}: Introducing the Mix-of-Expert structure can improve the \red{performance} and \red{generalization} of VLAs. \\
\midrule
\multirow{1}{*}{\textit{Q4}: When to Leverage \textbf{Extra Data}} & \textit{Q4}: Which training stage should introduce  \textcolor{red}{cross-embodiment} datasets? & \textit{A4}: 1) \textcolor{red}{Extra in-domain data} shows beneficial; 2) \textcolor{red}{Post-training} further improves high-frequency tasks as well as few-shot performance. \\
\bottomrule
\end{tabular}
\label{tab:chapter_split}
\end{extendedtable*}

\begin{extendedtable*}[!t]
\caption{Simulation performances on \textbf{CALVIN} benchmark, all models are trained on split ABCD/ABC, and evaluated on split D. KosMos P.H. represents the VLA utilizing KosMos-2 as backbone and policy head as architecture, built with the RoboVLMs framework, and is maximally trained for 5 epochs. We will continue to use the expression of backbone and structure to represent the VLAs built with RoboVLMs in the following paper. Note that KosMos refers to the VLM backbone we utilized, and ``P.H." refers to the policy head formulation.
}
\centering
% \begin{tabular}{l|c|c|ccccc|c}
\begin{tabularx}{\textwidth}{l@{\extracolsep{\fill}}|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X|>{\centering\arraybackslash}X} 
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{VLA?} & \multirow{2}{*}{Train} & \multicolumn{5}{c|}{Consecutive tasks success rates} & \multirow{2}{*}{\makecell{\textit{Avg.}\\\textit{Len.}}}  \\ \cmidrule{4-8} 
 &  &  & 1 & 2 & 3 & 4 & 5 &  \\ \hline
MCIL & \xmark & \multirow{8}{*}{ABCD} & 0.373 & 0.027 & 0.002 & 0.000 & 0.000 & 0.40 \\
R3M (Frozen) & \xmark &  & 0.085 & 0.005 & 0.001 & 0.000 & 0.000 & 0.10 \\
Voltron (Frozen) & \xmark &  & 0.101 & 0.003 & 0.001 & 0.000 & 0.000 & 0.11 \\
Voltron (Fine-tuned) & \xmark &  & 0.837 & 0.566 & 0.352 & 0.208 & 0.115 & 2.08 \\
RT-1 & \xmark &  & 0.844 & 0.617 & 0.438 & 0.323 & 0.227 & 2.45 \\
HULC & \xmark &  & 0.889 & 0.733 & 0.587 & 0.475 & 0.383 & 3.06 \\
% RoboFlamingo & Enc-Dec PH &  & 0.964 & 0.896 & 0.824 & 0.740 & 0.662 & 4.09 \\
GR-1 & \cmark &  & 0.949 & 0.896 & 0.844 & 0.789 & 0.731 & 4.21 \\
{KosMos P.H. (RoboVLMs)} & \cmark &  & {\bf 0.967} & {\bf 0.930} & {\bf 0.899} & {\bf 0.865} & {\bf 0.826} & {\bf 4.49} \\ \midrule %\hline \hline
MCIL & \xmark & \multirow{7}{*}{ABC} & 0.304 & 0.013 & 0.002 & 0.000 & 0.000 & 0.31 \\
Voltron (Frozen) & \xmark &  & 0.026 & 0.001 & 0.000 & 0.000 & 0.000 & 0.03 \\
Voltron (Fine-tuned)& \xmark &  & 0.569 & 0.272 & 0.105 & 0.038 & 0.014 & 1.00 \\
RT-1 & \xmark &  & 0.533 & 0.222 & 0.094 & 0.038 & 0.013 & 0.90 \\
HULC & \xmark &  & 0.418 & 0.165 & 0.057 & 0.019 & 0.011 & 0.67 \\
% RoboFlamingo &  &  & 0.824 & 0.619 & 0.466 & 0.331 & 0.235 & 2.48 \\
GR-1 & \cmark &  & 0.854 & 0.712 & 0.596 & 0.497 & 0.401 & 3.06 \\
{KosMos P.H. (RoboVLMs)} & \cmark &  & {\bf 0.980} & {\bf 0.936} & {\bf 0.854} & {\bf 0.778} & {\bf 0.704} & {\bf 4.25} \\ \bottomrule
\end{tabularx}
\label{tab:performance_calvin}
\end{extendedtable*}

\begin{extendedtable*}[!t]
    \centering
    \caption{The detailed performance on SimplerEnv.}
    \label{tab:simpler_merge}
    
    \begin{subtable}{\textwidth}
        \centering
        \caption{Simulation performance on \textbf{SimplerEnv}-\textit{WidowX+Bridge} environments. We report both the final success rates
(final) along with the sub-task success rates (e.g., \texttt{Grasp Spoon}).}
        \resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{\texttt{Put Spoon on Towel}} & \multicolumn{2}{c|}{\texttt{Put Carrot on Plate}} & \multicolumn{2}{c|}{\texttt{Stack Green Block on Yellow Block}} & \multicolumn{2}{c}{\texttt{Put Eggplant in Yellow Basket}} \\ \cmidrule{2-9} 
 & \texttt{Grasp Spoon} & final & \texttt{Grasp Carrot} & final & \texttt{Grasp Green Block} & final & \texttt{Grasp Eggplant} & final \\ \midrule
RT-1-X & 0.167 & 0.000 & 0.208 & 0.042 & 0.083 & 0.000 & 0.000 & 0.000 \\
Octo-Base & 0.347 & 0.125 & 0.528 & 0.083 & 0.319 & 0.000 & 0.667 & 0.431 \\
Octo-Small & {\bf 0.778} & {\bf 0.472} & 0.278 & 0.097 & 0.403 & 0.042 & 0.875 & 0.569 \\
OpenVLA-7b & 0.041 & 0.000 & 0.333 & 0.000 & 0.125 & 0.000 & 0.083 & 0.041 \\
% RoboVLMs (Bridge) & 0.583 & 0.500 & 0.500 & 0.292 & 0.625 & 0.125 & 0.583 & 0.500 \\
RoboVLMs (Ours) & 0.583 & 0.458 & {\bf 0.458} & {\bf 0.417} & {\bf 0.375} & {\bf 0.167} & {\bf 0.958} & {\bf 0.958} \\ \bottomrule
\end{tabular}
\vspace{-50pt}}
\label{tab:simpler_bridge}
    \end{subtable}
    
    \vspace{0.5cm}
    
    \begin{subtable}{\textwidth}
        \centering
        \caption{Simulation performance on \textbf{SimplerEnv}-\textit{Google Robot} environments.}
        \begin{tabularx}{\textwidth}{l|>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X|c|ccc|c}
\toprule
\multirow{4}{*}{Method} & \multicolumn{4}{c|}{\multirow{2}{*}{\texttt{Pick Coke Can}}} & \multirow{2}{*}{\texttt{Move Near}} & \multicolumn{3}{c|}{\multirow{2}{*}{\texttt{Open/Close Drawer}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{Open Top Drawer} \\ \texttt{and Place Apple} \end{tabular}} \\
 & \multicolumn{4}{c}{} &  & \multicolumn{3}{c}{} &  \\ \cmidrule{2-10} 
 & \begin{tabular}[c]{@{}c@{}}Horizontal\\ Laying\end{tabular} & \begin{tabular}[c]{@{}c@{}}Vertical\\ Laying\end{tabular} & Standing & Average & Average & Open & Close & Average & Average  \\ \midrule
RT-1 (Converged) & 0.960 & 0.900 & 0.710 & {\bf 0.857} & 0.442 & {\bf 0.601} & 0.861 & {\bf 0.730} & 0.000 \\
RT-1 ($15\%$) & 0.860 & 0.790 & 0.480 & 0.710 & 0.354 & 0.463 & 0.667 & 0.565 & 0.000 \\
RT-1-X & 0.820 & 0.330 & 0.550 & 0.567 & 0.317 & 0.296 & {\bf 0.891} & 0.597 & 0.213 \\
RT-2-X & 0.740 & 0.740 & 0.880 & 0.787 & 0.779 & 0.157 & 0.343 & 0.250 & 0.037 \\
Octo-Base & 0.210 & 0.210 & 0.090 & 0.170 & 0.042 & 0.009 & 0.444 & 0.227 & 0.000 \\
RT-1 (Begin) & 0.050 & 0.000 & 0.030 & 0.027 & 0.050 & 0.000 & 0.278 & 0.139 & 0.000 \\
OpenVLA-7b & 0.270 & 0.030 & 0.190 & 0.163 & 0.462 & 0.194 & 0.518 & 0.356 & 0.000 \\
RoboVLMs (Ours) & {\bf 1.000} & {\bf 0.910} & {\bf 1.000} & {\bf 0.970} & {\bf 0.888} & 0.565 & 0.537 & 0.551 & {\bf 0.325} \\ \bottomrule

\end{tabularx}
% \vspace{-50pt}
\label{tab:simpler_rt}
    \end{subtable}

    \vspace{0.5cm}
    
    \begin{subtable}{\textwidth}
        \centering
        \caption{Results on WidowX + Bridge setup for cross-embodiment dataset.}
        \resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{\texttt{Put Spoon on Towel}} & \multicolumn{2}{c|}{\texttt{Put Carrot on Plate}} & \multicolumn{2}{c|}{\texttt{Stack Green Block on Yellow Block}} & \multicolumn{2}{c}{\texttt{Put Eggplant in Yellow Basket}} \\ \cmidrule{2-9} 
 & \texttt{Grasp Spoon} & final & \texttt{Grasp Carrot} & final & \texttt{Grasp Green Block} & final & \texttt{Grasp Eggplant} & final \\ \midrule
% Target Task Finetune & 0.167 & 0.000 & 0.208 & 0.042 & 0.083 & 0.000 & 0.000 & 0.000 \\ In-domain Full Finetune
Cross-Emb Pre-Train & 0.458 & {\bf 0.458} & 0.333 & 0.250 & {\bf 0.458} & 0.042 & 0.916 & 0.833 \\
In-domain Full Finetune & {\bf 0.625} & 0.417 & 0.500 & 0.250 & 0.417 & 0.083 & {\bf 1.000} & {\bf 1.000} \\
Post Train & 0.583 & {\bf 0.458} & {\bf 0.458} &  {\bf 0.417} &  0.375 & {\bf 0.167} & 0.958 & 0.958 \\ 
\hline
\end{tabular}
% \vspace{-32pt}
\label{tab:cross_bridge}
}
    \end{subtable}

    \vspace{0.5cm}
    
    \begin{subtable}{\textwidth}
        \centering
        \caption{Results on WidowX + Bridge setup for cross-embodiment dataset.}
        \resizebox{\textwidth}{!}{
\begin{tabularx}{\textwidth}{l>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|ccc|cc}
\toprule
\multirow{4}{*}{Method} & \multicolumn{4}{c|}{\multirow{2}{*}{\texttt{Pick Coke Can}}} & \multirow{2}{*}{\texttt{Move Near}} & \multicolumn{3}{c|}{\multirow{2}{*}{\texttt{Open/Close Drawer}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{Open Top Drawer} \\ \texttt{and Place Apple} \end{tabular}} \\
 & \multicolumn{4}{c|}{} &  & \multicolumn{3}{c|}{} &  \\ \cmidrule{2-10} 
 & \begin{tabular}[c]{@{}c@{}}Horizontal\\ Laying\end{tabular} & \begin{tabular}[c]{@{}c@{}}Vertical\\ Laying\end{tabular} & Standing & Average & Average & Open & Close & Average & Average  \\ \midrule
Cross-Emb Pre-Train & 0.940 & 0.840 & 0.890 & 0.890 & 0.571 & 0.222 & 0.444 & 0.333 & 0.019 \\
Target Task Finetune & 0.420 & 0.320 & 0.440 & 0.400 & 0.448 & 0.167 & 0.567 & 0.368 & 0.000 \\
In-domain Full Finetune & {\bf 1.000} & 0.910 & {\bf 1.000} & 0.970 & {\bf 0.888} & {\bf 0.565} & 0.537 & {\bf 0.551} & {\bf 0.325} \\
Post Train & 0.990 & {\bf 0.960} & {\bf 1.000} & {\bf 0.980} & 0.740 & 0.250 & {\bf 0.670} & 0.460 & 0.050 \\ \hline
\end{tabularx}
% \vspace{-32pt}
% \vspace{-32pt}
\label{tab:cross_rt}
}
    \end{subtable}

    
\end{extendedtable*}

\begin{extendedtable*}[!t]
\caption{
The performance of VLAs implemented with different formulations and training data scales. The results for 0.1x and 1x data are the best-behaved model checkpoints within 5 epochs, and the results for 5x data are the model performance at 1\textsuperscript{st} epoch. We name different implemented VLAs by their VLM backbones and the way of history modeling. Results are reported with models trained maximally  within 5 epochs on the ABCD training splits.
}
\centering
% \begin{tabular}{l|c|ccccc|c}
\begin{tabularx}{\textwidth}{l@{\extracolsep{\fill}}|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X|>{\centering\arraybackslash}X} 
\toprule
\multirow{2}{*}{\makecell{VLA\\Architecture}} & \multirow{2}{*}{\makecell{Data\\Scale}} & \multicolumn{5}{c|}{Consecutive tasks success rates} & \multirow{2}{*}{\makecell{\textit{Avg.}\\\textit{Len.}}}\\ \cmidrule{3-7} 
 &  & 1 & 2 & 3 & 4 & 5 &  \\ \midrule
Flamingo P.H. 3B \quad & \multirow{5}{*}{0.1x} & 0.120 & 0.007  & 0.000  & 0.000  & 0.000  &  0.13\\
Flamingo P.H. 4B &  & 0.448 & 0.084  & 0.014  & 0.003  & 0.001  &  0.55\\
Flamingo P.H. 9B &  & 0.547   & 0.190  & 0.067  & 0.020  & 0.003  &  0.83 \\
% Flamingo P.H. 9B &  & 0.120 & 0.007  & 0.000  & 0.000  & 0.000  &  0.13 \\
% KosMos Inter. No VL &  &  \\
KosMos Inter. &  & 0.938 & 0.701 & 0.445 & 0.270 & 0.140 & 2.49 \\
% KosMos P.H. No VL &   \\
KosMos P.H. &  & 0.958 & 0.684 & 0.431 & 0.270 & 0.176 &  2.52 \\ \midrule
% KosMos P.H. (RTX Pre-Trained) &  & 0.905 & 0.643 & 0.430 & 0.274 & 0.186 & 2.44 \\ \hline \hline
Flamingo P.H. 3B & \multirow{5}{*}{1x} & 0.964 & 0.896 & 0.824 & 0.740 & 0.662 & 4.09\\
Flamingo P.H. 4B &  & 0.936 & 0.847 & 0.750 & 0.667 & 0.586 & 3.79\\
% Flamingo P.H. 9B No VL &  & 0.733 & 0.444 & 0.270 & 0.161 & 0.077 & 1.69 \\
Flamingo P.H. 9B &   & 0.955 & 0.879 & 0.784 & 0.714 & 0.634 & 3.97  \\
KosMos Inter. &  & 0.987 & 0.915 & 0.824 & 0.737 & 0.660 & 4.12 \\
KosMos P.H. &  & 0.967 & 0.930 & 0.899 & 0.865 & 0.826 & 4.49 \\ \midrule
Flamingo P.H. 3B & \multirow{3}{*}{5x} & 0.971 & 0.916 & 0.856 & 0.794 & 0.716 & 4.21 \\
KosMos Inter. &  & 0.989 & 0.940 & 0.892 & 0.842 & 0.795 & 4.46 \\
KosMos P.H. &  & 0.968 & 0.937 & 0.903 & 0.872 & 0.830 & 4.51 \\ \bottomrule
\end{tabularx}
\label{tab:data_eff_calvin}
\end{extendedtable*}

\begin{extendedtable*}[!t]
\caption{The performance of the built VLAs based on VLMs with different image token numbers and VL pre-train data scales. The first three rows are flamingo backbones with encoder-decoder structures, the rest backbones are decoder-only structures. Note that for VLMs with multi-stage training, the data scale refers to the data amount utilized for the final stage of fine-tuning. ``UNK'' denotes unknown. 
Results are reported with the model checkpoints trained with 5 epochs on the ABCD training splits, all models are trained with a single side view image for fair comparison. 
We surprisingly found that both LLaVA and Qwen behave badly without an additional resampler to downsample the number of tokens. 
}
\centering
% \begin{tabular}{l|ccc|ccccc|c}
\begin{tabularx}{\textwidth}{l@{\extracolsep{\fill}}|>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X|>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X|>{\centering\arraybackslash}X} 
\toprule
\multirow{2}{*}{Backbone} & \multirow{2}{*}{\#Token} & \multirow{2}{*}{\makecell{Data\\Scale}} & \multirow{2}{*}{\makecell{Model\\Size}} & \multicolumn{5}{c|}{Consecutive tasks success rates} & \multirow{2}{*}{\makecell{Avg.\\Len.}} \\ \cmidrule{5-9} 
 &  &  &  & 1 & 2 & 3 & 4 & 5 &  \\ \midrule
% LLaVA MPT & 196 & 0.5M & 7B &  &  &  &  &  & \\
% LLaVA Vicuna & 576 & 0.5M & 7B &  &  &  &  &  & \\
Flamingo & 64 & 1B+ & 3B & 0.692 & 0.418 & 0.241 & 0.14 & 0.074 & 1.57 \\
Flamingo & 64 & 1B+ & 4B & 0.689 & 0.456 & 0.281 & 0.181 & 0.107 & 1.71\\
Flamingo & 64 & 1B+ & 9B & 0.744 & 0.485 & 0.298 & 0.187 & 0.112 & 1.83\\ \midrule
Qwen-VL & 256 & 350K & 9B & 0.221 & 0.062 & 0.014 & 0.002 & 0.000 & 0.30 \\
MoonDream & 576 & UNK & 3B & 0.717 & 0.473 & 0.296 & 0.198 & 0.127 & 1.81 \\
Uform & 256 & 10M & 1.3B & 0.778 & 0.577 & 0.407 & 0.300 & 0.216 & 2.28 \\
% Cambrian & 224 & 10M & 3B &  &  &  &  &  &  \\
KosMos & 64 & 90M & 2B & 0.922 & 0.807 & 0.701 & 0.615 & 0.549 & 3.59 \\ 
Paligemma & 256 & 10B & 3B & 0.931 & 0.836 & 0.752 & 0.683 & 0.616 & 3.82 \\
\bottomrule
\end{tabularx}
\label{tab:calvin_backbone}
\end{extendedtable*}

\clearpage


==> papers/5-related.tex <==
\section{Preliminary and Method}\label{sec2}

\subsection{Imitation Learning}

Imitation learning, also known as programming by demonstrations, or learning from demonstrations~\citep{calinon2009robot, billard2008survey, argall2009survey}, provides a natural way to impart knowledge from human experts.
Some early works adopted symbolic reasoning upon the collected expert demonstrations~\citep{lozano1983robot, dufay1984approach, levas1984user}.
Limited by the model capacity and learning techniques, such methods decomposed demonstrations into motion or skill primitives to achieve corresponding subgoals~\citep{schaal2003computational, kober2009learning}.
% This idea is further combined with machine learning approaches to define and recognize elementary operators, based on which a basic motor skill library can be built~\citep{}.

In recent years, one of the most well-known ideas to learn from expert demonstrations is inverse reinforcement learning (IRL)~\citep{abbeel2004apprenticeship, arora2021survey, adams2022survey}.
As indicated by its name, the core technical challenge of IRL is to recover the underlying subtle reward function given the optimal behaviors collected by experts~\citep{abbeel2004apprenticeship}.
IRL is notoriously inefficient in terms of problem scale.
Though investigated broadly~\citep{aghasadeghi2011maximum, chan2021scalable, imani2021scalable, dexter2021inverse, chen2023fast}, IRL methods struggle to scale beyond limited state space and are mostly used to solve toy problems.
Besides, IRL typically involves iteratively learning rewards and RL policies, hence it is inefficient in learning efficiency and safety, which are undeniably required by robot learning.

Benefiting from vast progress in deep learning, behavioral cloning (BC) has shown the potential to solve complex manipulation problems~\citep{ross2011reduction, torabi2018behavioral, stepputtis2020language, jang2022bc}.
BC simply models the imitation learning problem as a standard supervised learning problem.
It assumes that one can get trajectories consisting of sequential observation-action pairs demonstrated by experts.
To learn from these demonstrations, the policy usually takes in the observations and is trained to map them directly to the corresponding actions.
Despite its simplicity, BC inherits the advantage of supervised learning, being scalable to large-scale problems and data~\citep{lin2024data, pearce2024scaling}.
Yet, it is data-intensive and its performance is highly subject to the training data~\citep{ren2021generalization, belkhale2024data, xie2024decomposing}.
To make BC more robust against diverse inputs, one well-known method, DAgger, introduces online learning with runtime expert demonstrations~\citep{ross2011reduction}.
% Therefore, when and how to ask for help is the key challenge for such kind of methods~\citep{}.
In summary, BC offers a straightforward and scalable approach to imitation learning, leveraging advances in deep learning to tackle complex manipulation tasks. 

\subsection{Pre-Training for Robot Manipulation}

Pre-training has been widely shown efficient to improve the data efficiency for vision and language tasks including language understanding~\citep{kenton2019bert, liu2019roberta} and generation~\citep{radford2019language, brown2020language}, image classification~\citep{deng2009imagenet, krizhevsky2012imagenet}, object detection~\citep{ren2016faster, redmon2016you, liu2016ssd} and segmentation~\citep{long2015fully, he2017mask}, captioning~\citep{vinyals2015show}, visual question answering~\citep{antol2015vqa}, etc. 
Recently, with the development of large-scale pre-trained models, imitation learning, especially behavioral cloning (BC), has shown promising results in inheriting knowledge from the pertaining stage and dataset~\citep{brohan2022rt, brohan2023rt, li2023vision, kim2024openvla}, which essentially helps the BC models to generalize across diverse visual and linguistic observations.

One conventional way to pre-train a deep neural network is supervised learning of image classification on the ImageNet dataset~\citep{deng2009imagenet}.
Recent works have demonstrated similar efficiency of using such pre-trained weights as the initiation of manipulation policies in robotic tasks, including grasping~\citep{redmon2015real, zhang2019real, asif2019densely}, navigation~\citep{gupta2017cognitive, zhu2017target}, and diverse household manipulation tasks~\citep{xiao2022masked, radosavovic2023real, radosavovic2023robot}.
To leverage pre-trained weights from ImageNet, intermediate representations for robotic tasks are typically formulated as computer vision tasks.
For example, grasping can be approximately formulated as a detection problem, with a grasp representation similar to object detection~\citep{redmon2015real} or segmentation~\citep{asif2019densely}.
Such an approximation, though losing generality to general robot skills, can sufficiently utilize the knowledge from pre-training and be more robust in application. 

Recently, vision-language representation learning has developed vastly and rapidly and has been shown to be efficient for downstream vision and language tasks~\citep{chen2023vlp, luo2020univl, lu2019vilbert, chen2020simple}.
Such models are usually trained on either the collection of diverse labeled datasets or unlabeled Internet-scale data.
They go beyond the knowledge of ImageNet and generalize well to open-world observations.
Therefore, such advanced pre-training techniques and models are explored as the foundation of downstream manipulation skills to improve robustness against open-world observations, including masked image and language modeling~\citep{he2022masked, karamcheti2023language, seo2023multi, wu2023masked}, contrastive learning~\citep{nair2022r3m, zhan2022learning, zhan2021framework, ma2021contrastive}, video analysis and understanding~\citep{ko2023learning, wen2023any, escontrela2024video}, video prediction~\citep{wu2023unleashing, cheang2024gr, du2024learning}, and vision-language pre-training~\citep{li2023vision, brohan2023rt, kim2024openvla}.
Specifically, temporal representations are crucial to learning skills involving sequential decision-making.
Hence, some works are well-known for enforcing the learned representations to encode temporal dynamics explicitly, ensuring that the model captures the progression of states over time~\citep{sermanet2018time, nair2022r3m}.
These advancements have demonstrated promising generality in handling partially observable real-world tasks.

In this paper, specifically, we investigate the effectiveness, efficiency, and generality of pre-trained large-scale vision-language models as the foundation of robotic manipulation skills.
We focus on the problem of:
\begin{itemize}
    \item What kind of pre-trained models are preferred
    \item How we formulate the problem of robotic manipulation given a pre-trained model.
    \item Why the preferred formulation works.
\end{itemize}
and try to 

\subsection{Language-Conditioned Robot Policies}

Languages are one of the most natural and user-friendly interfaces between robots and non-expert human users.
Therefore, it has been actively investigated to design language-instructed robot policies for a long history in human-robot interaction~\citep{goodrich2008human, sheridan2016human, zhou2023language}.
Early works, subject to the performance of language understanding models, usually design interaction templates for specific robotic tasks, including navigation~\citep{zelek1997human, levit2007interpretation, bonial2018human}, object manipulation~\citep{guadarrama2013grounding}, failure recovery~\citep{knepper2015recovering}, and disambiguation~\citep{fransen2007using, shridhar2020ingress, zhang2021invigorate}.
These methods typically model human-robot interaction with a finite set of interaction behaviors, extract environmental states from raw observations (e.g., vision and language inputs) explicitly, and develop probabilistic machine-learning models to map states to desired interactive actions.
However, limited by the capacity of the models, they are usually limited to processing relatively close-set and low-dimensional inputs, which restricts their performance when being deployed in realistic scenarios.

In recent years, deep learning models have enabled unified interfaces to process high-dimensional and diverse inputs~\citep{chen2022visuo, zhou2023visual, chen2024uamfdet}, especially visual images and natural language sequences~\citep{lu2019vilbert, alexey2020image}.
Therefore, the language-conditioned policy is becoming more and more popular and demonstrates promising results in designing robotic systems for non-expert users.
One of the most popular ways to develop language-conditioned policies is reinforcement learning (RL)~\citep{shao2021concept2robot, nair2022learning, peng2023conceptual}.
Typically, the policy includes a vision encoder, if any visual inputs, and a language encoder, which comprises either multi-layer perceptrons (MLP) and convolutional neural networks (CNN), or Transformer blocks, to extract vision-language embeddings.
A policy head is then trained with RL to map embeddings to robot actions, which are expected to maximize the cumulative rewards.
Yet, RL is known to be data-inefficient~\citep{li2017deep}.
Though lots of work has been devoted to higher data efficiency~\citep{kamthe2018data, nachum2018data, schwarzer2021pre-training, yu2018towards}, it still suffers from sim-to-real issues~\citep{zhao2020sim} and struggles with real-world deployment and learning to perform tasks with high complexity.

Recently, the most prevailing way to develop language-conditioned policies is through behavioral cloning (BC),  which directly maps visual and linguistic observations to expert actions~\citep{ross2011reduction, zare2024survey}. 
The key challenge is how to learn the joint representations for both visual and linguistic inputs to generalize well to diverse open-world environments and tasks, while keeping highly data-efficient with limited expert demonstrations.
Therefore, different kinds of feature learning and fusion strategies are proposed to solve this problem, like contrastive learning~\citep{nair2022r3m} and FiLM~\citep{perez2018film}.
Thanks to the Transformer network~\citep{vaswani2017attention}, it makes learning a shared space for vision and languages naturally no longer a problem.
By simply tokenizing input languages and visual images, Transformers formulate robot policy learning as a next token prediction problem conditioned on a sequence of visual and linguistic tokens~\citep{chen2021decision, brohan2023rt, driess2023palm, bousmalis2023robocat, wu2023unleashing, cheang2024gr}.
It has been broadly demonstrated to be convenient and useful in various robotic tasks.

\subsection{Generalist Robot Policies}

\subsection{Vision-Language-Action Models}

Recently, large language models (LLMs)~\citep{} have illustrated impressive power to process open-ended language expressions.
Hence, some approaches have exploited large language models (LLMs) as powerful task planners, to generate step-by-step plans on given tasks, subsequently instructing pre-trained low-level skills as executors~\citep{}.
Such policies decompose high-level symbolic planning and low-level control policies explicitly.
Though demonstrated to be useful in many cases, they suffer from problems of grounding to the real world due to the disability of seeing and reacting. 

To leverage the power of LLMs with visual inputs for multi-modal tasks, recent progress in multi-modal LLMs, or called large-scale vision-language models (VLMs), has proven the feasibility of directly learning a shared and aligned vision-language embedding space~\citep{}, with much less computational resources than pertaining a VLM from scratch.
These models have shown comparable reasoning ability in the aspect of commonsense knowledge from language pertaining while being able to accept visual inputs.
Based on the VLMs, one natural way to develop robot policies is to further train these models with downstream robot data~\citep{}.
Benefiting from the knowledge of the encyclopedic language repertoire during pre-training, such methods show surprising generality to ``unknown'' semantic inputs~\citep{}.
Such models are known as vision-language-action models (VLAs), since they can perform various vision-language-action tasks simultaneously.

To train such VLAs, a great variety of recipes have been proposed.
For training data, it is possible to further finetune the VLMs only with robot data~\citep{}, or joint vision-language-robot data~\citep{}.
For input formulation, single-image-based reactive policies~\citep{}, temporal observation sequences~\citep{}, and interleaved vision-language-action inputs~\citep{} are all shown to be feasible to learn reasonably good robot policies.
For actions, they can be democratized for the convenience of unified formulation with language tokens~\citep{}, or kept in continuous space for precise execution~\citep{}.
For policies, various powerful choices like Action Chunk Transformers~\citep{} and Diffusion Policies~\citep{} are proposed to improve robustness.
Moreover, various kinds of large-scale VLMs~\citep{} are emerging with new state-of-the-art performance on various vision-language benchmarks~\citep{}.
In this paper, we are investigating all the above great progress, to provide a comprehensive study of the key points to train a successful VLA. 




==> papers/7-avail.tex <==
\newpage
\section{Data availability}
Datasets used in this study could be found at \url{https://github.com/mees/calvin} (CALVIN), \url{https://github.com/google-deepmind/open_x_embodiment} (Open X-Embodiment), and \url{https://huggingface.co/datasets/robovlms/bytedance_robot_benchmark_20} (BDRBench20).

\section{Code availability}
The source code of this study could be found at \url{https://github.com/Robot-VLAs/RoboVLMs}.

==> tables/34_calvin_task_SR.tex <==

\begin{table*}[htbp]  
\caption{Sub-task level success rates by tasks in CALVIN under different VLM backbones.} 
\label{tb:task-res}
\centering  
\begin{tabularx}{\textwidth}{l|@{\extracolsep{\fill}}*{6}{c}} 
\toprule  
Task Name & Flamingo-3B & Flamingo-4B & Flamingo-9B & GR-1 & KosMos & MoonDream \\
\midrule
\texttt{rotate blue block right} & 0.947 & 0.893 & 0.729 & 0.770 & 0.493 & 0.882\\
\texttt{move slider right} & 0.996 & 0.993 & 0.996 & 0.992 & 0.987 & 0.996\\
\texttt{lift red block slider} & 0.890 & 0.970 & 0.967 & 0.858 & 0.856 & 0.927\\
\texttt{place in slider} & 0.904 & 0.828 & 0.582 & 0.911 & 0.874 & 0.910\\
\texttt{turn off lightbulb} & 0.972 & 1.000 & 0.992 & 0.956 & 0.927 & 0.964\\
\texttt{turn off led} & 0.988 & 1.000 & 1.000 & 0.994 & 0.970 & 0.981\\
\texttt{push into drawer} & 0.777 & 0.821 & 0.731 & 0.770 & 0.705 & 0.703\\
\texttt{lift blue block drawer} & 1.000 & 0.950 & 1.000 & 1.000 & 0.917 & 0.737\\
\texttt{close drawer} & 1.000 & 1.000 & 1.000 & 1.000 & 0.986 & 0.995\\
\texttt{lift pink block slider} & 0.940 & 0.971 & 0.944 & 0.862 & 0.861 & 0.918\\
\texttt{lift pink block table} & 0.859 & 0.851 & 0.905 & 0.892 & 0.543 & 0.899\\
\texttt{move slider left} & 0.996 & 0.996 & 1.000 & 1.000 & 0.970 & 0.996\\
\texttt{open drawer} & 0.976 & 0.997 & 0.997 & 0.982 & 0.980 & 0.997\\
\texttt{turn on lightbulb} & 0.988 & 0.994 & 1.000 & 0.988 & 0.949 & 0.988\\
\texttt{rotate blue block left} & 0.923 & 0.939 & 0.820 & 0.925 & 0.636 & 0.848\\
\texttt{push blue block left} & 0.746 & 0.955 & 0.841 & 0.836 & 0.677 & 0.909\\
\texttt{rotate red block right} & 0.926 & 0.972 & 0.853 & 0.905 & 0.591 & 0.959\\
\texttt{turn on led} & 0.988 & 0.988 & 0.994 & 0.976 & 0.985 & 0.994\\
\texttt{push pink block right} & 0.652 & 0.754 & 0.833 & 0.651 & 0.627 & 0.750\\
\texttt{push red block left} & 0.949 & 0.920 & 0.849 & 0.949 & 0.562 & 0.908\\
\texttt{lift blue block table} & 0.891 & 0.956 & 0.925 & 0.927 & 0.611 & 0.931\\
\texttt{place in drawer} & 0.988 & 0.989 & 0.988 & 0.975 & 0.971 & 0.976\\
\texttt{rotate red block left} & 0.970 & 0.908 & 0.950 & 0.953 & 0.677 & 0.952\\
\texttt{push pink block left} & 0.947 & 0.920 & 0.915 & 0.973 & 0.747 & 0.933\\
\texttt{stack block} & 0.612 & 0.641 & 0.608 & 0.595 & 0.569 & 0.604\\
\texttt{lift blue block slider} & 0.847 & 0.963 & 0.908 & 0.826 & 0.769 & 0.869\\
\texttt{push red block right} & 0.657 & 0.732 & 0.797 & 0.451 & 0.457 & 0.653\\
\texttt{lift red block table} & 0.948 & 0.939 & 0.942 & 0.975 & 0.606 & 0.989\\
\texttt{lift pink block drawer} & 0.857 & 0.800 & 0.929 & 0.714 & 0.778 & 0.923\\
\texttt{rotate pink block right} & 0.917 & 0.896 & 0.714 & 0.794 & 0.478 & 0.789\\
\texttt{unstack block} & 1.000 & 0.982 & 0.957 & 0.980 & 0.946 & 0.979\\
\texttt{rotate pink block left} & 0.929 & 0.839 & 0.906 & 0.818 & 0.698 & 0.927\\
\texttt{push blue block right} & 0.479 & 0.597 & 0.471 & 0.478 & 0.400 & 0.594\\
\texttt{lift red block drawer} & 0.947 & 1.000 & 1.000 & 1.000 & 0.769 & 0.933 \\
 \bottomrule  
\end{tabularx}
\end{table*}

==> tables/ablation_vlm_pretrain1.tex <==
\begin{table*}[!t]\tiny
\caption{Ablation of Vision-Langauge Pretrain.
}
\centering
\resizebox{\textwidth}{!}{
% \begin{tabular}{lccccccc}
\begin{tabularx}{\textwidth}{l@{\extracolsep{\fill}}*{7}{c}} 
\hline
\multirow{2}{*}{Backbone} & \multirow{2}{*}{Pretrained?} & \multicolumn{6}{c}{Tasks completed in a row} \\ \cmidrule{3-8} 
 &  & 1 & 2 & 3 & 4 & 5 & Avg Len \\ \hline
% Enc-Dec & N& 0.1x &  \\
% Enc-Dec & Y& 0.1x & 0.120 & 0.007  & 0.000  & 0.000  & 0.000  &  0.13 \\
% Dec-only & N& 0.1x &  \\
% Dec-only & Y& 0.1x & 0.958 & 0.684 & 0.431 & 0.270 & 0.176 &  2.52 \\ \hline \hline
% Dec-only PH (RTX Pre-Trained) & 0.1x & 0.905 & 0.643 & 0.430 & 0.274 & 0.186 & 2.44 \\ \hline \hline
\multirow{2}{*}{LLaVA} & N& &  \\
 & Y  \\ \hline 
\multirow{2}{*}{Flamingo} & N& &  \\
 & Y & 0.964 & 0.896 & 0.824 & 0.740 & 0.662 & 4.09 \\ \hline 
\multirow{2}{*}{KOSMOS} & N &  \\
 & Y & 0.967 & 0.930 & 0.899 & 0.865 & 0.826 & 4.49 \\ \hline% \hline

% Enc-Dec & N& 5x &  \\
% Enc-Dec & Y& 5x & 0.971 & 0.916 & 0.856 & 0.794 & 0.716 & 4.21 \\
% Dec-only & N& 5x &  \\
% Dec-only & Y& 5x & 0.968 & 0.937 & 0.903 & 0.872 & 0.830 & 4.51 \\ \hline
\end{tabularx}
\label{tab:pretrain_abl}
}
\end{table*}


==> tables/compare_robovlm_calvin.tex <==
\begin{table*}[!t]
\caption{Performance on CALVIN benchmark, all models are trained on split ABCD/ABC, and evaluated on split D. Results are reported using the best-behaved model checkpoints.
}
\centering
% \begin{tabular}{l|cccccccc}
% \begin{tabularx}{\textwidth}{l@{\extracolsep{\fill}}|cccccccc} 
\begin{tabularx}{\textwidth}{|l|*{8}{>{\centering\arraybackslash}X|}}
\toprule
\multirow{2}{*}{Structure} & \multirow{2}{*}{Train} & \multicolumn{5}{c}{Consecutive tasks success rates} & \multirow{2}{*}{\makecell{\textit{Avg.}\\\textit{Len.}}} \\ \cmidrule{3-7} 
 &  & 1 & 2 & 3 & 4 & 5 &  \\ \midrule
 Enc-Dec PH 3B & \multirow{6}{*}{ABCD} & 0.964 & 0.896 & 0.824 & 0.740 & 0.662 & 4.09 \\
 Enc-Dec PH 4B &  & 0.936 & 0.847 & 0.750 & 0.667 & 0.586 & 3.79 \\
 Enc-Dec PH 9B No VL &  & 0.733 & 0.444 & 0.270 & 0.161 & 0.077 & 1.69  \\
 Enc-Dec PH 9B &  & 0.955 & 0.879 & 0.784 & 0.714 & 0.634 & 3.97 \\
 Dec-only Inter &  & 0.987 & 0.915 & 0.824 & 0.737 & 0.660 & 4.12 \\
 Dec-only PH &  & 0.967 & 0.930 & 0.899 & 0.865 & 0.826 & 4.49 \\ \midrule
 Enc-Dec PH 3B & \multirow{4}{*}{ABC} & 0.829 & 0.636 & 0.453 & 0.321 & 0.234 & 2.47 \\
 % Enc-Dec PH 4B & ABC  \\
 % Enc-Dec PH 9B No VL & ABC &  \\
 Enc-Dec PH 9B &  & 0.758 & 0.574 & 0.392 & 0.288 & 0.188 & 2.20 \\
 Dec-only Inter &  & 0.824 & 0.684 & 0.524 & 0.376 & 0.296 & 2.70 \\
 Dec-only PH &  & 0.980 & 0.936 & 0.854 & 0.778 & 0.704 & 4.25 \\ \bottomrule
\end{tabularx}
\label{tab:calvin_perf_gen}
\end{table*}


==> tables/cross_emb.tex <==
\begin{table*}[htbp]
\caption{SimplerEnv simulation evaluation results for the WidowX + Bridge setup.
}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{\texttt{Put Spoon on Towel}} & \multicolumn{2}{c|}{\texttt{Put Carrot on Plate}} & \multicolumn{2}{c|}{\texttt{Stack Green Block on Yellow Block}} & \multicolumn{2}{c}{\texttt{Put Eggplant in Yellow Basket}} \\ \cmidrule{2-9} 
 & \texttt{Grasp Spoon} & final & \texttt{Grasp Carrot} & final & \texttt{Grasp Green Block} & final & \texttt{Grasp Eggplant} & final \\ \midrule
% Target Task Finetune & 0.167 & 0.000 & 0.208 & 0.042 & 0.083 & 0.000 & 0.000 & 0.000 \\ In-domain Full Finetune
Cross-Emb Pre-Train & 0.458 & {\bf 0.458} & 0.333 & 0.250 & {\bf 0.458} & 0.042 & 0.916 & 0.833 \\
In-domain Full Finetune & {\bf 0.625} & 0.417 & 0.500 & 0.250 & 0.417 & 0.083 & {\bf 1.000} & {\bf 1.000} \\
Post Train & 0.583 & {\bf 0.458} & {\bf 0.458} &  {\bf 0.417} &  0.375 & {\bf 0.167} & 0.958 & 0.958 \\ 
\hline
\end{tabular}
% \vspace{-32pt}
\label{tab:cross_bridge}
}
\end{table*}



\begin{table*}[htbp]
\caption{SimplerEnv simulator evaluation results across different policies on Google Robot tasks.}
\centering
\begin{tabularx}{\textwidth}{l>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|ccc|cc}
\toprule
\multirow{4}{*}{Method} & \multicolumn{4}{c|}{\multirow{2}{*}{\texttt{Pick Coke Can}}} & \multirow{2}{*}{\texttt{Move Near}} & \multicolumn{3}{c|}{\multirow{2}{*}{\texttt{Open/Close Drawer}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{Open Top Drawer} \\ \texttt{and Place Apple} \end{tabular}} \\
 & \multicolumn{4}{c|}{} &  & \multicolumn{3}{c|}{} &  \\ \cmidrule{2-10} 
 & \begin{tabular}[c]{@{}c@{}}Horizontal\\ Laying\end{tabular} & \begin{tabular}[c]{@{}c@{}}Vertical\\ Laying\end{tabular} & Standing & Average & Average & Open & Close & Average & Average  \\ \midrule
Cross-Emb Pre-Train & 0.940 & 0.840 & 0.890 & 0.890 & 0.571 & 0.222 & 0.444 & 0.333 & 0.019 \\
Target Task Finetune & 0.420 & 0.320 & 0.440 & 0.400 & 0.448 & 0.167 & 0.567 & 0.368 & 0.000 \\
In-domain Full Finetune & {\bf 1.000} & 0.910 & {\bf 1.000} & 0.970 & {\bf 0.888} & {\bf 0.565} & 0.537 & {\bf 0.551} & {\bf 0.325} \\
Post Train & 0.990 & {\bf 0.960} & {\bf 1.000} & {\bf 0.980} & 0.740 & 0.250 & {\bf 0.670} & 0.460 & 0.050 \\ \hline
\end{tabularx}
% \vspace{-32pt}
\label{tab:cross_rt}
\end{table*}


==> tables/data_efficiency_novl.tex <==
\begin{extendedtable*}[!t]\tiny
\caption{Data Efficiency of Models with or without Vision-Language Pretrain on CALVIN benchmark. The results for 0.1x and 1x data are the best-behaved model checkpoints within 5 epochs, and the results for 5x data are the model performance at 1 epoch.
}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccccc}
\toprule
\multirow{2}{*}{Structure} & \multirow{2}{*}{Data Scale} & \multicolumn{5}{c}{Tasks completed in a sequence} & \multirow{2}{*}{Avg. Len.}\\ \cmidrule{3-7} 
 &  & 1 & 2 & 3 & 4 & 5 &  \\ \hline
Dec-only Inter No VL & 1x & 0.692 & 0.382 & 0189 & 0.085 & 0.036 & 1.38 \\
Dec-only Inter & 1x & 0.987 & 0.915 & 0.824 & 0.737 & 0.660 & 4.12 \\
Dec-only PH No VL & 1x & 0.815 & 0.626 & 0.473 & 0.349 & 0.245 & 2.51 \\
Dec-only PH & 1x & 0.967 & 0.930 & 0.899 & 0.865 & 0.826 & 4.49 \\ \midrule
% Enc-Dec PH 4B & 5x \\
% Enc-Dec PH 9B No VL & 5x  \\
% Enc-Dec PH 9B & 5x & \\
Dec-only Inter No VL & 5x & 0.833 & 0.588 & 0.421 & 0.297 & 0.209 & 2.35\\
Dec-only Inter & 5x & 0.989 & 0.940 & 0.892 & 0.842 & 0.795 & 4.46 \\
Dec-only PH No VL & 5x & 0.893 & 0.755 & 0.644 & 0.564 & 0.462 & 3.32 \\
Dec-only PH & 5x & 0.968 & 0.937 & 0.903 & 0.872 & 0.830 & 4.51 \\ \bottomrule
\end{tabular}
\label{tab:data_eff_novl_calvin}
}
\end{extendedtable*}


==> tables/flamingo_backbone.tex <==
\begin{table*}[!t]\tiny
\caption{The performance on 10\% language annotated data on $ABCD\rightarrow D$ setting for different Flamingo Model backbone with Policy Head formulation. All variants are trained and evaluated for the same training epochs.}
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Backbone} & \multicolumn{6}{c}{Task Completed in a Sequence (Success Rate)} \\ 
                        & 1      & 2     & 3     & 4     & 5     & Avg Len \\ \hline
MPT-3B                   & 0.047   & 0.003  & 0.000  & 0.000  & 0.000  &  0.05       \\ 
MPT-3B-IFT                   & 0.120   & 0.007  & 0.000  & 0.000  & 0.000  &  0.13       \\ 
GPT-Neox-4B                   & 0.420   & 0.054  & 0.003  & 0.000  & 0.000  &  0.48       \\ 
GPT-Neox-4B-IFT                   & 0.448   & 0.084  & 0.014  & 0.003  & 0.001  &  0.55       \\ 
% L-9B                   & 0.499   & 0.149  & 0.036  & 0.011  & 0.001  &  0.69       \\ \hline
MPT-9B                   & 0.547   & 0.190  & 0.067  & 0.020  & 0.003  &  0.83      \\ \bottomrule
\end{tabular}
\label{tab:flamingo_data_eff}
}
\end{table*}

==> tables/pali_moe.tex <==
\begin{table*}[!t]
\caption{
The effectiveness of the Mix-of-Expert structure with different training objectives. We utilize PaliGemma, which aligns with the settings of $\pi$ series, as the VLM backbone and implement Fully Connecting (FC) with MSE and Flow Matching (FM) loss. Note that the FC with Flow Matching loss and MoE structure is identity with $\pi_0$, and for fair comparison, we do not consider state as input.
}
\centering
% \begin{tabular}{l|c|ccccc|c}
\begin{tabularx}{\textwidth}{l@{\extracolsep{\fill}}|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X|>{\centering\arraybackslash}X} 
\toprule
\multirow{2}{*}{\makecell{Training\\Objective}} & \multirow{2}{*}{\makecell{Using\\MoE}} & \multicolumn{5}{c|}{Consecutive tasks success rates} & \multirow{2}{*}{\makecell{\textit{Avg.}\\\textit{Len.}}}\\ \cmidrule{3-7} 
 &  & 1 & 2 & 3 & 4 & 5 &  \\ \midrule
MSE+BCE & \checkmark (ABC) & 0.932 & 0.824 & 0.732 & 0.644 & 0.556 & 3.69   \\
MSE+BCE & \ding{55} (ABC) & 0.901 & 0.802 & 0.703 & 0.620 & 0.544 & 3.57 \\
Flow Matching \ \ & \checkmark (ABC) & 0.940 & 0.855 & 0.768 & 0.679  & 0.597  & 3.84   \\
Flow Matching \ \  & \ding{55} (ABC) & 0.910 & 0.812 & 0.730 & 0.652 & 0.573 & 3.68 \\ 
\midrule
MSE+BCE & \checkmark (ABCD) & 0.945 & 0.823 & 0.678 & 0.561 & 0.457 & 3.46  \\
MSE+BCE & \ding{55} (ABCD) & 0.933 & 0.863 & 0.808 & 0.751 & 0.688 & 4.04 \\
Flow Matching \ \ & \checkmark (ABCD) & 0.911 & 0.828 & 0.759 & 0.707 & 0.639 & 3.84 \\
Flow Matching \ \  & \ding{55} (ABCD) & 0.937 & 0.872 &  0.811 & 0.764 & 0.705 & 4.10 \\

\bottomrule
\end{tabularx}
\label{tab:moe}
\end{table*}


==> tables/simpler_bridge.tex <==
\begin{table*}[htbp]
\caption{Simulation performance on \textbf{SimplerEnv}-\textit{WidowX+Bridge} environments. We report both the final success rates
(final) along with the sub-task success rates (e.g., \texttt{Grasp Spoon}).
}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{\texttt{Put Spoon on Towel}} & \multicolumn{2}{c|}{\texttt{Put Carrot on Plate}} & \multicolumn{2}{c|}{\texttt{Stack Green Block on Yellow Block}} & \multicolumn{2}{c}{\texttt{Put Eggplant in Yellow Basket}} \\ \cmidrule{2-9} 
 & \texttt{Grasp Spoon} & final & \texttt{Grasp Carrot} & final & \texttt{Grasp Green Block} & final & \texttt{Grasp Eggplant} & final \\ \midrule
RT-1-X & 0.167 & 0.000 & 0.208 & 0.042 & 0.083 & 0.000 & 0.000 & 0.000 \\
Octo-Base & 0.347 & 0.125 & 0.528 & 0.083 & 0.319 & 0.000 & 0.667 & 0.431 \\
Octo-Small & {\bf 0.778} & {\bf 0.472} & 0.278 & 0.097 & 0.403 & 0.042 & 0.875 & 0.569 \\
OpenVLA-7b & 0.041 & 0.000 & 0.333 & 0.000 & 0.125 & 0.000 & 0.083 & 0.041 \\
% RoboVLMs (Bridge) & 0.583 & 0.500 & 0.500 & 0.292 & 0.625 & 0.125 & 0.583 & 0.500 \\
RoboVLMs (Ours) & 0.583 & 0.458 & {\bf 0.458} & {\bf 0.417} & {\bf 0.375} & {\bf 0.167} & {\bf 0.958} & {\bf 0.958} \\ \bottomrule
\end{tabular}
\vspace{-50pt}
\label{tab:simpler_bridge}
}
\end{table*}

==> tables/simpler_rt.tex <==

\begin{table*}[htbp]
\caption{Simulation performance on \textbf{SimplerEnv}-\textit{Google Robot} environments.}
\centering
\begin{tabularx}{\textwidth}{l|>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X|c|ccc|c}
\toprule
\multirow{4}{*}{Method} & \multicolumn{4}{c|}{\multirow{2}{*}{\texttt{Pick Coke Can}}} & \multirow{2}{*}{\texttt{Move Near}} & \multicolumn{3}{c|}{\multirow{2}{*}{\texttt{Open/Close Drawer}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\texttt{Open Top Drawer} \\ \texttt{and Place Apple} \end{tabular}} \\
 & \multicolumn{4}{c}{} &  & \multicolumn{3}{c}{} &  \\ \cmidrule{2-10} 
 & \begin{tabular}[c]{@{}c@{}}Horizontal\\ Laying\end{tabular} & \begin{tabular}[c]{@{}c@{}}Vertical\\ Laying\end{tabular} & Standing & Average & Average & Open & Close & Average & Average  \\ \midrule
RT-1 (Converged) & 0.960 & 0.900 & 0.710 & {\bf 0.857} & 0.442 & {\bf 0.601} & 0.861 & {\bf 0.730} & 0.000 \\
RT-1 ($15\%$) & 0.860 & 0.790 & 0.480 & 0.710 & 0.354 & 0.463 & 0.667 & 0.565 & 0.000 \\
RT-1-X & 0.820 & 0.330 & 0.550 & 0.567 & 0.317 & 0.296 & {\bf 0.891} & 0.597 & 0.213 \\
RT-2-X & 0.740 & 0.740 & 0.880 & 0.787 & 0.779 & 0.157 & 0.343 & 0.250 & 0.037 \\
Octo-Base & 0.210 & 0.210 & 0.090 & 0.170 & 0.042 & 0.009 & 0.444 & 0.227 & 0.000 \\
RT-1 (Begin) & 0.050 & 0.000 & 0.030 & 0.027 & 0.050 & 0.000 & 0.278 & 0.139 & 0.000 \\
OpenVLA-7b & 0.270 & 0.030 & 0.190 & 0.163 & 0.462 & 0.194 & 0.518 & 0.356 & 0.000 \\
RoboVLMs (Ours) & {\bf 1.000} & {\bf 0.910} & {\bf 1.000} & {\bf 0.970} & {\bf 0.888} & 0.565 & 0.537 & 0.551 & {\bf 0.325} \\ \bottomrule

\end{tabularx}
% \vspace{-50pt}
\label{tab:simpler_rt}
\end{table*}



==> tables/train_loss.tex <==
\begin{table*}[!t]
\caption{
The performance of VLAs implemented with different training objective. All VLAs utilize PaliGemma as VLM backbone and takes only the current observation as input (\texttt{One-Step-Continuous} model). While at each time step the VLA outputs an action chunk, we verify three different action executing paradigms: {\bf Chunk} represents that the VLAs execute the entire chunk. {\bf First} refers to VLAs execute the first action in the chunk. {\bf Ensemble} refers to ensemble the first action with the corresponding actions in history chunks. All models are trained on ABC splits and tested on D split with PaliGemma backbone.
}
\centering
% \begin{tabular}{l|c|c|ccccc|c}
\begin{tabularx}{\textwidth}{l@{\extracolsep{\fill}}|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X|>{\centering\arraybackslash}X} 
\toprule
\multirow{2}{*}{\makecell{Training\\Objective}} & \multirow{2}{*}{\makecell{Training\\Split}} & \multirow{2}{*}{\makecell{Executing\\Paradigm}} & \multicolumn{5}{c|}{Consecutive tasks success rates} & \multirow{2}{*}{\makecell{\textit{Avg.}\\\textit{Len.}}}\\ \cmidrule{4-8} 
 &  &  & 1 & 2 & 3 & 4 & 5 &  \\ \midrule
% DDPM  & Chunk  & 0.863  & 0.620  & 0.417  & 0.273  & 0.168 & 2.34 \\
% DDPM & First & 0.613  &  0.264 & 0.090  & 0.025  & 0.008 & 1.00 \\
% DDPM & Ensemble & 0.834  & 0.512  & 0.305  & 0.174  & 0.101 & 1.93 \\ \midrule
Flow Matching\ \  & \multirow{6}{*}{ABC}  & Chunk & 0.910 & 0.812 & 0.730 & 0.652 & 0.573 & 3.68 \\
Flow Matching\ \  & & First  & 0.793  & 0.586  & 0.442  & 0.351  & 0.273 & 2.45 \\
Flow Matching\ \  & & Ensemble  & 0.838  & 0.710  & 0.614  & 0.545  & 0.437 & 3.14 \\ 
% \midrule
MSE+BCE  & & Chunk  & 0.901 & 0.802 & 0.703 & 0.620 & 0.544 & 3.57 \\
MSE+BCE & & First  & 0.822  & 0.564  & 0.371  & 0.265  & 0.169 & 2.19 \\
MSE+BCE & & Ensemble  & 0.880  & 0.730  & 0.606  & 0.508  & 0.414 & 3.14 \\ 
\midrule
% DDPM (Chunk) & \multirow{9}{*}{ABCD}  &   &   &   &   &  & \\
% DDPM (First) &  &   &   &   &   &  & \\
% DDPM (Ensemble) &  &   &   &   &   &  & \\
Flow Matching\ \  & \multirow{6}{*}{ABCD}  & Chunk  & 0.937 & 0.872 &  0.811 & 0.764 & 0.705 & 4.09 \\
Flow Matching\ \ &  & First  & 0.898  & 0.799 & 0.701 & 0.618 & 0.544 & 3.56 \\
Flow Matching\ \ & & Ensemble &  0.945 & 0.882  & 0.818  & 0.770  & 0.708 & 4.12\\
MSE+BCE  & & Chunk  & 0.933 & 0.863 & 0.808 & 0.751 & 0.688 & 4.04 \\
MSE+BCE & & First  & 0.925 & 0.727 & 0.579 &  0.473 & 0.378 & 3.06 \\
MSE+BCE & & Ensemble  &  0.925 & 0.849 & 0.784  & 0.721  & 0.664 & 3.94 \\ 

\bottomrule
\end{tabularx}
\label{tab:train_loss}
\end{table*}
